Amplituhedra and origami, II: loop level

Building on the recently discovered origami-amplituhedron correspondence, we prove that the BCFW (Britto-Cachazo-Feng-Witten) cells triangulate the $m=4$ amplituhedron in full generality at all loop orders, both in momentum and momentum-twistor space. Along the way, we develop two natural "$L$-punctured" extensions of the positive Grassmannian and relate them via T-duality.

==> t_embeddings_v2_aux.tex <==
\relax 
\providecommand \babel@aux [2]{\global \let \babel@toc \@gobbletwo }
\@nameuse{bbl@beforestart}
\providecommand\hyper@newdestlabel[2]{}
\providecommand\HyField@AuxAddToFields[1]{}
\providecommand\HyField@AuxAddToCoFields[2]{}
\citation{Hull}
\citation{Hull}
\citation{origami2}
\citation{BCFW}
\citation{AHT}
\citation{Hodges}
\babel@aux{english}{}
\@writefile{toc}{\contentsline {section}{\tocsection {}{}{Introduction}}{1}{section*.3}\protected@file@percent }
\citation{AHT}
\citation{ELT}
\citation{ELPTSBW}
\citation{DFLP}
\citation{FL}
\citation{abcgpt}
\citation{LPW}
\citation{ELT}
\citation{ELPTSBW}
\citation{ELT}
\citation{ELPTSBW}
\citation{AHT}
\citation{AHTT}
\citation{AHTT}
\citation{ELPTSBW}
\citation{Hull}
\citation{KLRR}
\citation{CLR1}
\citation{Kawasaki}
\citation{Hull}
\citation{KLRR}
\citation{CLR1}
\citation{Smirnov_cluster}
\citation{CheSmi}
\@writefile{lof}{\contentsline {figure}{\numberline {1}{\ignorespaces An origami crease pattern $\hat  {\bm  {x}}(\Gamma ^\ast )$ (left) and its image $\check  {\bm  {x}}(\Gamma ^\ast )$ under the origami map (right). The Kawasaki angle\xspace  condition is satisfied at each interior vertex of $\hat  {\bm  {x}}(\Gamma ^\ast )$, which allows it to be folded consistently. Figure reproduced from~\cite  [Figure~1]{Hull}.}}{2}{figure.caption.2}\protected@file@percent }
\newlabel{fig:orig}{{1}{2}{An origami crease pattern $\Tcal (\GD )$ (left) and its image $\Ocal (\GD )$ under the origami map (right). The \Kawangle condition is satisfied at each interior vertex of $\Tcal (\GD )$, which allows it to be folded consistently. Figure reproduced from~\cite [Figure~1]{Hull}}{figure.caption.2}{}}
\newlabel{fig:orig@cref}{{[figure][1][]1}{[1][1][]2}{}{}{}}
\@writefile{loe}{\contentsline {theoremintro}{\ifthmt@listswap Theorem~A\else \numberline {A}Theorem\fi }{2}{theoremintro.1}\protected@file@percent }
\newlabel{thm:intro:A}{{A}{2}{}{theoremintro.1}{}}
\newlabel{thm:intro:A@cref}{{[theoremintro][1][]A}{[1][2][]2}{}{}{}}
\citation{Chelkak_ICM}
\citation{Chelkak_s_emb}
\citation{KLRR}
\citation{CLR1}
\citation{CLR2}
\citation{BNR}
\citation{KLRR}
\citation{Pos}
\citation{origami2}
\citation{origami2}
\citation{Lus2}
\citation{Pos}
\citation{KLRR}
\citation{CLR1}
\citation{Kenyon}
\citation{AHCC}
\citation{abcgpt}
\citation{abcgpt}
\citation{MuSp}
\citation{DFLP}
\@writefile{loe}{\contentsline {theoremintro}{\ifthmt@listswap Theorem~B\else \numberline {B}Theorem\fi }{3}{theoremintro.2}\protected@file@percent }
\newlabel{thm:intro:B}{{B}{3}{}{theoremintro.2}{}}
\newlabel{thm:intro:B@cref}{{[theoremintro][2][]B}{[1][3][]3}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\tocsubsection {}{}{Changelog}}{3}{section*.4}\protected@file@percent }
\citation{origami2}
\citation{Huang_Wen}
\citation{Chelkak_s_emb}
\citation{Lovasz_Plummer}
\citation{Pos}
\@writefile{toc}{\contentsline {section}{\tocsection {}{1}{Main results}}{4}{section.1}\protected@file@percent }
\newlabel{sec:main_results}{{1}{4}{Main results}{section.1}{}}
\newlabel{sec:main_results@cref}{{[section][1][]1}{[1][4][]4}{}{}{}}
\newlabel{sec:intro:plabic}{{1.1}{4}{Background on total positivity and the dimer model}{subsection.1.1}{}}
\newlabel{sec:intro:plabic@cref}{{[subsection][1][1]1.1}{[1][4][]4}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\tocsubsection {}{1.1}{Background on total positivity and the dimer model}}{4}{subsection.1.1}\protected@file@percent }
\newlabel{eq:intro:Delta_G_wt}{{1.1}{4}{Background on total positivity and the dimer model}{equation.1.1}{}}
\newlabel{eq:intro:Delta_G_wt@cref}{{[equation][1][1]1.1}{[1][4][]4}{}{}{}}
\newlabel{eq:DIM:helWmin_dfn}{{1.2}{4}{Background on total positivity and the dimer model}{equation.1.2}{}}
\newlabel{eq:DIM:helWmin_dfn@cref}{{[equation][2][1]1.2}{[1][4][]4}{}{}{}}
\newlabel{eq:surplus_dfn}{{1.3}{4}{Background on total positivity and the dimer model}{equation.1.3}{}}
\newlabel{eq:surplus_dfn@cref}{{[equation][3][1]1.3}{[1][4][]4}{}{}{}}
\citation{KLRR}
\citation{CLR1}
\citation{KLRR}
\citation{KLRR}
\newlabel{eq:intro:Grnd_dfn}{{1.4}{5}{Background on total positivity and the dimer model}{equation.1.4}{}}
\newlabel{eq:intro:Grnd_dfn@cref}{{[equation][4][1]1.4}{[1][5][]5}{}{}{}}
\newlabel{sec:intro:t_emb}{{1.2}{5}{T-embeddings and t-immersions}{subsection.1.2}{}}
\newlabel{sec:intro:t_emb@cref}{{[subsection][2][1]1.2}{[1][5][]5}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\tocsubsection {}{1.2}{T-embeddings and t-immersions}}{5}{subsection.1.2}\protected@file@percent }
\newlabel{eq:intro:wtT_dfn}{{1.5}{5}{T-embeddings and t-immersions}{equation.1.5}{}}
\newlabel{eq:intro:wtT_dfn@cref}{{[equation][5][1]1.5}{[1][5][]5}{}{}{}}
\newlabel{eq:intro:gauge}{{1.6}{5}{T-embeddings and t-immersions}{equation.1.6}{}}
\newlabel{eq:intro:gauge@cref}{{[equation][6][1]1.6}{[1][5][]5}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~1.1\else \numberline {1.1}Definition\fi }{5}{definition.1.1}\protected@file@percent }
\newlabel{dfn:intro:sum_angles}{{1.1}{5}{}{definition.1.1}{}}
\newlabel{dfn:intro:sum_angles@cref}{{[definition][1][1]1.1}{[1][5][]5}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~1.2\else \numberline {1.2}Definition\fi \thmtformatoptarg {\cite  {KLRR,CLR1}}}{5}{definition.1.2}\protected@file@percent }
\newlabel{dfn:intro:t_imm}{{1.2}{5}{\cite {KLRR,CLR1}}{definition.1.2}{}}
\newlabel{dfn:intro:t_imm@cref}{{[definition][2][1]1.2}{[1][5][]5}{}{}{}}
\newlabel{intro:t_imm_straight_convex}{{{{(TE1)}}}{5}{\cite {KLRR,CLR1}}{Item.1}{}}
\newlabel{intro:t_imm_straight_convex@cref}{{[enumi][1][]{{(TE1)}}}{[1][5][]5}{}{}{}}
\newlabel{intro:t_imm_orientation}{{{{(TE2)}}}{5}{\cite {KLRR,CLR1}}{Item.2}{}}
\newlabel{intro:t_imm_orientation@cref}{{[enumi][2][]{{(TE2)}}}{[1][5][]5}{}{}{}}
\newlabel{intro:t_imm_gauge}{{{{(TE3)}}}{5}{\cite {KLRR,CLR1}}{Item.3}{}}
\newlabel{intro:t_imm_gauge@cref}{{[enumi][3][]{{(TE3)}}}{[1][5][]5}{}{}{}}
\newlabel{intro:t_imm_angles_int}{{{{(TE4)}}}{5}{\cite {KLRR,CLR1}}{Item.4}{}}
\newlabel{intro:t_imm_angles_int@cref}{{[enumi][4][]{{(TE4)}}}{[1][5][]5}{}{}{}}
\newlabel{eq:intro:t_imm_angles_int}{{1.7}{5}{\cite {KLRR,CLR1}}{equation.1.7}{}}
\newlabel{eq:intro:t_imm_angles_int@cref}{{[equation][7][1]1.7}{[1][5][]5}{}{}{}}
\newlabel{intro:t_imm_angles_bdry}{{{{(TE5)}}}{5}{\cite {KLRR,CLR1}}{Item.5}{}}
\newlabel{intro:t_imm_angles_bdry@cref}{{[enumi][5][]{{(TE5)}}}{[1][5][]5}{}{}{}}
\newlabel{eq:intro:t_imm_angles_bdry}{{1.8}{5}{\cite {KLRR,CLR1}}{equation.1.8}{}}
\newlabel{eq:intro:t_imm_angles_bdry@cref}{{[equation][8][1]1.8}{[1][5][]5}{}{}{}}
\citation{AHTT}
\@writefile{lof}{\contentsline {figure}{\numberline {2}{\ignorespaces  A t-embedding (left) and a t-immersion (right).}}{6}{figure.caption.5}\protected@file@percent }
\newlabel{fig:t-imm}{{2}{6}{A t-embedding (left) and a t-immersion (right)}{figure.caption.5}{}}
\newlabel{fig:t-imm@cref}{{[figure][2][]2}{[1][5][]6}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\tocsubsection {}{1.3}{Origami-amplituhedron correspondence\xspace  }}{6}{subsection.1.3}\protected@file@percent }
\newlabel{eq:intro:LALATS}{{1.9}{6}{\OACTITLE }{equation.1.9}{}}
\newlabel{eq:intro:LALATS@cref}{{[equation][9][1]1.9}{[1][5][]6}{}{}{}}
\newlabel{eq:intro:wind}{{1.10}{6}{\OACTITLE }{equation.1.10}{}}
\newlabel{eq:intro:wind@cref}{{[equation][10][1]1.10}{[1][6][]6}{}{}{}}
\newlabel{eq:intro:LALAK}{{1.11}{6}{\OACTITLE }{equation.1.11}{}}
\newlabel{eq:intro:LALAK@cref}{{[equation][11][1]1.11}{[1][6][]6}{}{}{}}
\newlabel{eq:intro:TRIPLES}{{1.12}{6}{\OACTITLE }{equation.1.12}{}}
\newlabel{eq:intro:TRIPLES@cref}{{[equation][12][1]1.12}{[1][6][]6}{}{}{}}
\@writefile{loe}{\contentsline {theorem}{\ifthmt@listswap Theorem~1.3\else \numberline {1.3}Theorem\fi \thmtformatoptarg {Origami-amplituhedron correspondence\xspace  }}{6}{theorem.1.3}\protected@file@percent }
\newlabel{thm:intro:t_imm_vs_triples}{{1.3}{6}{\OACTITLE }{theorem.1.3}{}}
\newlabel{thm:intro:t_imm_vs_triples@cref}{{[theorem][3][1]1.3}{[1][6][]6}{}{}{}}
\citation{CLR1}
\citation{KLRR}
\citation{DFLP}
\citation{KLRR}
\citation{KLRR}
\citation{origami2}
\@writefile{lof}{\contentsline {figure}{\numberline {3}{\ignorespaces  When $(\Lambda ,\tilde  \Lambda )$ is $\breve  {\mathbb  {A}}$-representable\xspace  , the momentum amplituhedron map $\Phi _{\Lambda ,\tilde  \Lambda }$ corresponds to gluing an annular graph $\breve  {\Gamma }$ to the boundary of $\Gamma $; see \cref  {ssec:annular}. }}{7}{figure.caption.6}\protected@file@percent }
\newlabel{fig:intro-annular}{{3}{7}{When $\LaLat $ is \Arep , the momentum amplituhedron map $\PhiLL $ corresponds to gluing an annular graph $\Gbot $ to the boundary of $\G $; see \cref {ssec:annular}}{figure.caption.6}{}}
\newlabel{fig:intro-annular@cref}{{[figure][3][]3}{[1][7][]7}{}{}{}}
\newlabel{sec:intro:mom}{{1.4}{7}{Momentum amplituhedron}{subsection.1.4}{}}
\newlabel{sec:intro:mom@cref}{{[subsection][4][1]1.4}{[1][7][]7}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\tocsubsection {}{1.4}{Momentum amplituhedron}}{7}{subsection.1.4}\protected@file@percent }
\newlabel{eq:intro:LaLat}{{1.13}{7}{Momentum amplituhedron}{equation.1.13}{}}
\newlabel{eq:intro:LaLat@cref}{{[equation][13][1]1.13}{[1][7][]7}{}{}{}}
\newlabel{eq:intro:PhiLL_dfn}{{1.14}{7}{Momentum amplituhedron}{equation.1.14}{}}
\newlabel{eq:intro:PhiLL_dfn@cref}{{[equation][14][1]1.14}{[1][7][]7}{}{}{}}
\@writefile{loe}{\contentsline {corollary}{\ifthmt@listswap Corollary~1.4\else \numberline {1.4}Corollary\fi }{7}{corollary.1.4}\protected@file@percent }
\@writefile{loe}{\contentsline {remark}{\ifthmt@listswap Remark~1.5\else \numberline {1.5}Remark\fi }{7}{remark.1.5}\protected@file@percent }
\newlabel{rmk:KLRR}{{1.5}{7}{}{remark.1.5}{}}
\newlabel{rmk:KLRR@cref}{{[remark][5][1]1.5}{[1][7][]7}{}{}{}}
\citation{DFLP}
\citation{CLR1}
\citation{HZ_notes}
\citation{DFLP}
\citation{DHKS}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~1.6\else \numberline {1.6}Definition\fi \thmtformatoptarg {\cite  {DFLP}}}{8}{definition.1.6}\protected@file@percent }
\newlabel{dfn:intro:MomLL}{{1.6}{8}{\cite {DFLP}}{definition.1.6}{}}
\newlabel{dfn:intro:MomLL@cref}{{[definition][6][1]1.6}{[1][8][]8}{}{}{}}
\newlabel{eq:intro:MomLL_dfn}{{1.15}{8}{\cite {DFLP}}{equation.1.15}{}}
\newlabel{eq:intro:MomLL_dfn@cref}{{[equation][15][1]1.15}{[1][8][]8}{}{}{}}
\@writefile{loe}{\contentsline {remark}{\ifthmt@listswap Remark~1.7\else \numberline {1.7}Remark\fi }{8}{remark.1.7}\protected@file@percent }
\newlabel{rmk:dim_MomLL}{{1.7}{8}{}{remark.1.7}{}}
\newlabel{rmk:dim_MomLL@cref}{{[remark][7][1]1.7}{[1][8][]8}{}{}{}}
\newlabel{sec:intro:origami_mand}{{1.5}{8}{Origami map and Mandelstam variables}{subsection.1.5}{}}
\newlabel{sec:intro:origami_mand@cref}{{[subsection][5][1]1.5}{[1][8][]8}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\tocsubsection {}{1.5}{Origami map and Mandelstam variables}}{8}{subsection.1.5}\protected@file@percent }
\newlabel{eq:intro:O_preserves_edges}{{1.16}{8}{Origami map and Mandelstam variables}{equation.1.16}{}}
\newlabel{eq:intro:O_preserves_edges@cref}{{[equation][16][1]1.16}{[1][8][]8}{}{}{}}
\newlabel{eq:intro:1_Lipschitz}{{1.17}{8}{Origami map and Mandelstam variables}{equation.1.17}{}}
\newlabel{eq:intro:1_Lipschitz@cref}{{[equation][17][1]1.17}{[1][8][]8}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~1.8\else \numberline {1.8}Definition\fi }{8}{definition.1.8}\protected@file@percent }
\newlabel{dfn:intro:1_Lipschitz}{{1.8}{8}{}{definition.1.8}{}}
\newlabel{dfn:intro:1_Lipschitz@cref}{{[definition][8][1]1.8}{[1][8][]8}{}{}{}}
\newlabel{eq:intro:Mand_dfn}{{1.18}{8}{Origami map and Mandelstam variables}{equation.1.18}{}}
\newlabel{eq:intro:Mand_dfn@cref}{{[equation][18][1]1.18}{[1][8][]8}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~1.9\else \numberline {1.9}Definition\fi }{8}{definition.1.9}\protected@file@percent }
\newlabel{eq:intro:M_amb_dfn}{{1.19}{8}{Origami map and Mandelstam variables}{equation.1.19}{}}
\newlabel{eq:intro:M_amb_dfn@cref}{{[equation][19][1]1.19}{[1][8][]8}{}{}{}}
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~1.10\else \numberline {1.10}Lemma\fi }{8}{lemma.1.10}\protected@file@percent }
\newlabel{lemma:intro:Mand_vs_norm}{{1.10}{8}{}{lemma.1.10}{}}
\newlabel{lemma:intro:Mand_vs_norm@cref}{{[lemma][10][1]1.10}{[1][8][]8}{}{}{}}
\newlabel{eq:intro:Mand_vs_norm}{{1.20}{8}{}{equation.1.20}{}}
\newlabel{eq:intro:Mand_vs_norm@cref}{{[equation][20][1]1.20}{[1][8][]8}{}{}{}}
\citation{DFLP}
\citation{RhSk}
\citation{Lam_dimers}
\citation{BCFW}
\citation{ELT}
\citation{AHT}
\citation{ELPTSBW}
\@writefile{loe}{\contentsline {remark}{\ifthmt@listswap Remark~1.11\else \numberline {1.11}Remark\fi }{9}{remark.1.11}\protected@file@percent }
\newlabel{rmk:intro:Minkowski}{{1.11}{9}{}{remark.1.11}{}}
\newlabel{rmk:intro:Minkowski@cref}{{[remark][11][1]1.11}{[1][8][]9}{}{}{}}
\newlabel{eq:inv_null}{{1.21}{9}{Origami map and Mandelstam variables}{equation.1.21}{}}
\newlabel{eq:inv_null@cref}{{[equation][21][1]1.21}{[1][9][]9}{}{}{}}
\@writefile{loe}{\contentsline {theorem}{\ifthmt@listswap Theorem~1.12\else \numberline {1.12}Theorem\fi }{9}{theorem.1.12}\protected@file@percent }
\newlabel{thm:intro:Mand_pos_exists}{{1.12}{9}{}{theorem.1.12}{}}
\newlabel{thm:intro:Mand_pos_exists@cref}{{[theorem][12][1]1.12}{[1][9][]9}{}{}{}}
\@writefile{loe}{\contentsline {corollary}{\ifthmt@listswap Corollary~1.13\else \numberline {1.13}Corollary\fi }{9}{corollary.1.13}\protected@file@percent }
\newlabel{cor:intro:t_emb_exists}{{1.13}{9}{}{corollary.1.13}{}}
\newlabel{cor:intro:t_emb_exists@cref}{{[corollary][13][1]1.13}{[1][9][]9}{}{}{}}
\newlabel{sec:intro:BCFW}{{1.6}{9}{\ORATITLE and BCFW tilings}{subsection.1.6}{}}
\newlabel{sec:intro:BCFW@cref}{{[subsection][6][1]1.6}{[1][9][]9}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\tocsubsection {}{1.6}{Origami reconstruction algorithm\xspace  and BCFW tilings}}{9}{subsection.1.6}\protected@file@percent }
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~1.14\else \numberline {1.14}Definition\fi }{9}{definition.1.14}\protected@file@percent }
\newlabel{dfn:intro:triang}{{1.14}{9}{}{definition.1.14}{}}
\newlabel{dfn:intro:triang@cref}{{[definition][14][1]1.14}{[1][9][]9}{}{}{}}
\newlabel{intro:triang1}{{{{(a)}}}{9}{}{Item.6}{}}
\newlabel{intro:triang1@cref}{{[enumi][1][]{{(a)}}}{[1][9][]9}{}{}{}}
\newlabel{intro:triang2}{{{{(b)}}}{9}{}{Item.7}{}}
\newlabel{intro:triang2@cref}{{[enumi][2][]{{(b)}}}{[1][9][]9}{}{}{}}
\newlabel{intro:triang3}{{{{(c)}}}{9}{}{Item.8}{}}
\newlabel{intro:triang3@cref}{{[enumi][3][]{{(c)}}}{[1][9][]9}{}{}{}}
\@writefile{loe}{\contentsline {theorem}{\ifthmt@listswap Theorem~1.15\else \numberline {1.15}Theorem\fi }{9}{theorem.1.15}\protected@file@percent }
\newlabel{thm:intro:BCFW}{{1.15}{9}{}{theorem.1.15}{}}
\newlabel{thm:intro:BCFW@cref}{{[theorem][15][1]1.15}{[1][9][]9}{}{}{}}
\@writefile{loe}{\contentsline {remark}{\ifthmt@listswap Remark~1.16\else \numberline {1.16}Remark\fi }{9}{remark.1.16}\protected@file@percent }
\@writefile{lof}{\contentsline {figure}{\numberline {4}{\ignorespaces  Applying a step of the BCFW recursion (left) and of the origami reconstruction algorithm\xspace  (right), recovering the point $\hat  {\bm  {x}}(\tilde  {f}^{\ast })=\check  {\bm  {x}}(\tilde  {f}^{\ast })$ as the intersection of $\ell _{{j_0}}$ and $\hat  {{\mathfrak  {R}}}$; see \cref  {sec:intro:BCFW}.}}{10}{figure.caption.7}\protected@file@percent }
\newlabel{fig:BCFW}{{4}{10}{Applying a step of the BCFW recursion (left) and of the \ora (right), recovering the point $\xTout (\fo )=\xOout (\fo )$ as the intersection of $\line _\jo $ and $\ray $; see \cref {sec:intro:BCFW}}{figure.caption.7}{}}
\newlabel{fig:BCFW@cref}{{[figure][4][]4}{[1][10][]10}{}{}{}}
\newlabel{lalat_bdry1}{{{{(i)}}}{10}{\ORATITLE and BCFW tilings}{Item.9}{}}
\newlabel{lalat_bdry1@cref}{{[enumi][1][]{{(i)}}}{[1][10][]10}{}{}{}}
\newlabel{lalat_bdry2}{{{{(ii)}}}{10}{\ORATITLE and BCFW tilings}{Item.10}{}}
\newlabel{lalat_bdry2@cref}{{[enumi][2][]{{(ii)}}}{[1][10][]10}{}{}{}}
\newlabel{lalat_bdry3}{{{{(iii)}}}{10}{\ORATITLE and BCFW tilings}{Item.11}{}}
\newlabel{lalat_bdry3@cref}{{[enumi][3][]{{(iii)}}}{[1][10][]10}{}{}{}}
\citation{BCFW}
\citation{BCFW}
\citation{Valentine}
\citation{Akop_Tar}
\citation{Tasmuratov}
\citation{Pak_book}
\citation{KLRR}
\citation{CLR1}
\citation{AGPR}
\@writefile{loe}{\contentsline {remark}{\ifthmt@listswap Remark~1.17\else \numberline {1.17}Remark\fi }{11}{remark.1.17}\protected@file@percent }
\@writefile{loe}{\contentsline {remark}{\ifthmt@listswap Remark~1.18\else \numberline {1.18}Remark\fi }{11}{remark.1.18}\protected@file@percent }
\newlabel{sec:intro:holomorphic}{{1.7}{11}{\KSprims }{subsection.1.7}{}}
\newlabel{sec:intro:holomorphic@cref}{{[subsection][7][1]1.7}{[1][11][]11}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\tocsubsection {}{1.7}{Kenyon--Smirnov primitives\xspace  }}{11}{subsection.1.7}\protected@file@percent }
\newlabel{eq:intro:white_holom}{{1.22}{11}{\KSprims }{equation.1.22}{}}
\newlabel{eq:intro:white_holom@cref}{{[equation][22][1]1.22}{[1][11][]11}{}{}{}}
\newlabel{eq:intro:holom_C_and_Cp}{{1.23}{11}{\KSprims }{equation.1.23}{}}
\newlabel{eq:intro:holom_C_and_Cp@cref}{{[equation][23][1]1.23}{[1][11][]11}{}{}{}}
\citation{CLR2}
\citation{Huang_Wen}
\citation{Huang_Wen_Xie}
\citation{Chelkak_s_emb}
\citation{applets}
\citation{KLRR}
\citation{CLR1}
\citation{CLR2}
\citation{applets}
\newlabel{eq:intro:primitive_TO}{{1.24}{12}{\KSprims }{equation.1.24}{}}
\newlabel{eq:intro:primitive_TO@cref}{{[equation][24][1]1.24}{[1][11][]12}{}{}{}}
\newlabel{eq:intro:y_to_lalat}{{1.25}{12}{\KSprims }{equation.1.25}{}}
\newlabel{eq:intro:y_to_lalat@cref}{{[equation][25][1]1.25}{[1][12][]12}{}{}{}}
\newlabel{eq:intro:Fw_Fb_y}{{1.26}{12}{\KSprims }{equation.1.26}{}}
\newlabel{eq:intro:Fw_Fb_y@cref}{{[equation][26][1]1.26}{[1][12][]12}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\tocsubsection {}{1.8}{Outline}}{12}{subsection.1.8}\protected@file@percent }
\@writefile{toc}{\contentsline {subsection}{\tocsubsection {}{}{Acknowledgments}}{12}{section*.8}\protected@file@percent }
\@writefile{toc}{\contentsline {section}{\tocsection {}{2}{Preliminaries}}{12}{section.2}\protected@file@percent }
\newlabel{sec:backgr}{{2}{12}{Preliminaries}{section.2}{}}
\newlabel{sec:backgr@cref}{{[section][2][]2}{[1][12][]12}{}{}{}}
\newlabel{sec:backgr:plabic}{{2.1}{12}{Planar bipartite graphs}{subsection.2.1}{}}
\newlabel{sec:backgr:plabic@cref}{{[subsection][1][2]2.1}{[1][12][]12}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\tocsubsection {}{2.1}{Planar bipartite graphs}}{12}{subsection.2.1}\protected@file@percent }
\newlabel{eq:DIM:k_dfn}{{2.1}{12}{Planar bipartite graphs}{equation.2.1}{}}
\newlabel{eq:DIM:k_dfn@cref}{{[equation][1][2]2.1}{[1][12][]12}{}{}{}}
\citation{Pos}
\citation{LamCDM}
\citation{KLS}
\citation{KLS}
\newlabel{eq:Euler_no_float}{{2.2}{13}{Planar bipartite graphs}{equation.2.2}{}}
\newlabel{eq:Euler_no_float@cref}{{[equation][2][2]2.2}{[1][12][]13}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~2.1\else \numberline {2.1}Definition\fi }{13}{definition.2.1}\protected@file@percent }
\newlabel{dfn:DIM:GD}{{2.1}{13}{}{definition.2.1}{}}
\newlabel{dfn:DIM:GD@cref}{{[definition][1][2]2.1}{[1][13][]13}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~2.2\else \numberline {2.2}Definition\fi }{13}{definition.2.2}\protected@file@percent }
\newlabel{dfn:positroid_Grneck}{{2.2}{13}{}{definition.2.2}{}}
\newlabel{dfn:positroid_Grneck@cref}{{[definition][2][2]2.2}{[1][13][]13}{}{}{}}
\newlabel{sec:backgr:Grtnn}{{2.2}{13}{Totally nonnegative Grassmannian}{subsection.2.2}{}}
\newlabel{sec:backgr:Grtnn@cref}{{[subsection][2][2]2.2}{[1][13][]13}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\tocsubsection {}{2.2}{Totally nonnegative Grassmannian}}{13}{subsection.2.2}\protected@file@percent }
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~2.3\else \numberline {2.3}Definition\fi }{13}{definition.2.3}\protected@file@percent }
\newlabel{dfn:bound_kn}{{2.3}{13}{}{definition.2.3}{}}
\newlabel{dfn:bound_kn@cref}{{[definition][3][2]2.3}{[1][13][]13}{}{}{}}
\newlabel{eq:gr_neck_dfn}{{2.3}{13}{Totally nonnegative Grassmannian}{equation.2.3}{}}
\newlabel{eq:gr_neck_dfn@cref}{{[equation][3][2]2.3}{[1][13][]13}{}{}{}}
\newlabel{eq:dfn_fC}{{2.4}{13}{Totally nonnegative Grassmannian}{equation.2.4}{}}
\newlabel{eq:dfn_fC@cref}{{[equation][4][2]2.4}{[1][13][]13}{}{}{}}
\newlabel{eq:Ptp_intersection}{{2.5}{13}{Totally nonnegative Grassmannian}{equation.2.5}{}}
\newlabel{eq:Ptp_intersection@cref}{{[equation][5][2]2.5}{[1][13][]13}{}{}{}}
\newlabel{eq:Ptp_vs_Meas}{{2.6}{13}{Totally nonnegative Grassmannian}{equation.2.6}{}}
\newlabel{eq:Ptp_vs_Meas@cref}{{[equation][6][2]2.6}{[1][13][]13}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~2.4\else \numberline {2.4}Definition\fi }{13}{definition.2.4}\protected@file@percent }
\newlabel{dfn:reduced}{{2.4}{13}{}{definition.2.4}{}}
\newlabel{dfn:reduced@cref}{{[definition][4][2]2.4}{[1][13][]13}{}{}{}}
\citation{Kasteleyn}
\citation{AGPR}
\citation{SpeyerVariations}
\citation{Kasteleyn}
\citation{TF_exact}
\citation{AGPR}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~2.5\else \numberline {2.5}Definition\fi }{14}{definition.2.5}\protected@file@percent }
\newlabel{dfn:top_cell_graph}{{2.5}{14}{}{definition.2.5}{}}
\newlabel{dfn:top_cell_graph@cref}{{[definition][5][2]2.5}{[1][14][]14}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~2.6\else \numberline {2.6}Definition\fi }{14}{definition.2.6}\protected@file@percent }
\newlabel{dfn:perfect_orient}{{2.6}{14}{}{definition.2.6}{}}
\newlabel{dfn:perfect_orient@cref}{{[definition][6][2]2.6}{[1][14][]14}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~2.7\else \numberline {2.7}Definition\fi }{14}{definition.2.7}\protected@file@percent }
\newlabel{dfn:nondeg}{{2.7}{14}{}{definition.2.7}{}}
\newlabel{dfn:nondeg@cref}{{[definition][7][2]2.7}{[1][14][]14}{}{}{}}
\newlabel{ssec:Kast_KSprims}{{2.3}{14}{Kasteleyn theory and \KSprims }{subsection.2.3}{}}
\newlabel{ssec:Kast_KSprims@cref}{{[subsection][3][2]2.3}{[1][14][]14}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\tocsubsection {}{2.3}{Kasteleyn theory and Kenyon--Smirnov primitives\xspace  }}{14}{subsection.2.3}\protected@file@percent }
\newlabel{eq:h_Path_dfn}{{2.7}{14}{Kasteleyn theory and \KSprims }{equation.2.7}{}}
\newlabel{eq:h_Path_dfn@cref}{{[equation][7][2]2.7}{[1][14][]14}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~2.8\else \numberline {2.8}Definition\fi \thmtformatoptarg {\cite  {AGPR,SpeyerVariations}}}{14}{definition.2.8}\protected@file@percent }
\newlabel{dfn:DIM:Kast}{{2.8}{14}{\cite {AGPR,SpeyerVariations}}{definition.2.8}{}}
\newlabel{dfn:DIM:Kast@cref}{{[definition][8][2]2.8}{[1][14][]14}{}{}{}}
\newlabel{eq:Kast_sign}{{2.8}{14}{\cite {AGPR,SpeyerVariations}}{equation.2.8}{}}
\newlabel{eq:Kast_sign@cref}{{[equation][8][2]2.8}{[1][14][]14}{}{}{}}
\@writefile{loe}{\contentsline {remark}{\ifthmt@listswap Remark~2.9\else \numberline {2.9}Remark\fi }{14}{remark.2.9}\protected@file@percent }
\newlabel{rmk:DIM:Kast_sign_bdfn}{{2.9}{14}{}{remark.2.9}{}}
\newlabel{rmk:DIM:Kast_sign_bdfn@cref}{{[remark][9][2]2.9}{[1][14][]14}{}{}{}}
\@writefile{loe}{\contentsline {remark}{\ifthmt@listswap Remark~2.10\else \numberline {2.10}Remark\fi }{14}{remark.2.10}\protected@file@percent }
\newlabel{rmk:Kast_sign_float}{{2.10}{14}{}{remark.2.10}{}}
\newlabel{rmk:Kast_sign_float@cref}{{[remark][10][2]2.10}{[1][14][]14}{}{}{}}
\citation{Kenyon_lectures}
\citation{AGPR}
\citation{AGPR}
\citation{AGPR}
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~2.11\else \numberline {2.11}Lemma\fi }{15}{lemma.2.11}\protected@file@percent }
\newlabel{lemma:OCP:Kast_even}{{2.11}{15}{}{lemma.2.11}{}}
\newlabel{lemma:OCP:Kast_even@cref}{{[lemma][11][2]2.11}{[1][14][]15}{}{}{}}
\newlabel{eq:partial_F_dfn}{{2.9}{15}{Kasteleyn theory and \KSprims }{equation.2.9}{}}
\newlabel{eq:partial_F_dfn@cref}{{[equation][9][2]2.9}{[1][15][]15}{}{}{}}
\newlabel{eq:TE:t_imm_bdry_vs_pFw_pFb}{{2.10}{15}{Kasteleyn theory and \KSprims }{equation.2.10}{}}
\newlabel{eq:TE:t_imm_bdry_vs_pFw_pFb@cref}{{[equation][10][2]2.10}{[1][15][]15}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~2.12\else \numberline {2.12}Definition\fi }{15}{definition.2.12}\protected@file@percent }
\newlabel{dfn:MCE:WKmat}{{2.12}{15}{}{definition.2.12}{}}
\newlabel{dfn:MCE:WKmat@cref}{{[definition][12][2]2.12}{[1][15][]15}{}{}{}}
\@writefile{loe}{\contentsline {proposition}{\ifthmt@listswap Proposition~2.13\else \numberline {2.13}Proposition\fi \thmtformatoptarg {\cite  {AGPR}}}{15}{proposition.2.13}\protected@file@percent }
\newlabel{lemma:MCE:Delta_vs_Kast}{{2.13}{15}{\cite {AGPR}}{proposition.2.13}{}}
\newlabel{lemma:MCE:Delta_vs_Kast@cref}{{[proposition][13][2]2.13}{[1][15][]15}{}{}{}}
\@writefile{loe}{\contentsline {corollary}{\ifthmt@listswap Corollary~2.14\else \numberline {2.14}Corollary\fi }{15}{corollary.2.14}\protected@file@percent }
\newlabel{lemma:MCE:apm_vs_Kast}{{2.14}{15}{}{corollary.2.14}{}}
\newlabel{lemma:MCE:apm_vs_Kast@cref}{{[corollary][14][2]2.14}{[1][15][]15}{}{}{}}
\newlabel{apm_vs_Kast1}{{{{(1)}}}{15}{}{Item.12}{}}
\newlabel{apm_vs_Kast1@cref}{{[enumi][1][]{{(1)}}}{[1][15][]15}{}{}{}}
\newlabel{apm_vs_Kast2}{{{{(2)}}}{15}{}{Item.13}{}}
\newlabel{apm_vs_Kast2@cref}{{[enumi][2][]{{(2)}}}{[1][15][]15}{}{}{}}
\newlabel{apm_vs_Kast3}{{{{(3)}}}{15}{}{Item.14}{}}
\newlabel{apm_vs_Kast3@cref}{{[enumi][3][]{{(3)}}}{[1][15][]15}{}{}{}}
\newlabel{eq:MCE:alt(C)_vs_pFw}{{2.11}{15}{}{equation.2.11}{}}
\newlabel{eq:MCE:alt(C)_vs_pFw@cref}{{[equation][11][2]2.11}{[1][15][]15}{}{}{}}
\@writefile{loe}{\contentsline {remark}{\ifthmt@listswap Remark~2.15\else \numberline {2.15}Remark\fi }{15}{remark.2.15}\protected@file@percent }
\newlabel{rmk:MCE:BKmat}{{2.15}{15}{}{remark.2.15}{}}
\newlabel{rmk:MCE:BKmat@cref}{{[remark][15][2]2.15}{[1][15][]15}{}{}{}}
\newlabel{eq:MCE:alt(Cp)_vs_pFb}{{2.12}{15}{}{equation.2.12}{}}
\newlabel{eq:MCE:alt(Cp)_vs_pFb@cref}{{[equation][12][2]2.12}{[1][15][]15}{}{}{}}
\@writefile{loe}{\contentsline {proposition}{\ifthmt@listswap Proposition~2.16\else \numberline {2.16}Proposition\fi }{15}{proposition.2.16}\protected@file@percent }
\newlabel{lemma:DIM:remove_bivertex}{{2.16}{15}{}{proposition.2.16}{}}
\newlabel{lemma:DIM:remove_bivertex@cref}{{[proposition][16][2]2.16}{[1][15][]15}{}{}{}}
\newlabel{eq:DIM:remove_bivertex_w}{{2.13}{15}{}{equation.2.13}{}}
\newlabel{eq:DIM:remove_bivertex_w@cref}{{[equation][13][2]2.13}{[1][15][]15}{}{}{}}
\newlabel{eq:DIM:remove_bivertex_b}{{2.14}{15}{}{equation.2.14}{}}
\newlabel{eq:DIM:remove_bivertex_b@cref}{{[equation][14][2]2.14}{[1][15][]15}{}{}{}}
\citation{BHL}
\citation{Kenyon_lectures}
\@writefile{lof}{\contentsline {figure}{\numberline {5}{\ignorespaces Examples of discrete holomorphic functions.}}{16}{figure.caption.9}\protected@file@percent }
\newlabel{fig:holom}{{5}{16}{Examples of discrete holomorphic functions}{figure.caption.9}{}}
\newlabel{fig:holom@cref}{{[figure][5][]5}{[1][16][]16}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~2.17\else \numberline {2.17}Definition\fi \thmtformatoptarg {Boundary restriction and extension}}{16}{definition.2.17}\protected@file@percent }
\newlabel{dfn:OCP:restr_ext}{{2.17}{16}{Boundary restriction and extension}{definition.2.17}{}}
\newlabel{dfn:OCP:restr_ext@cref}{{[definition][17][2]2.17}{[1][16][]16}{}{}{}}
\@writefile{loe}{\contentsline {example}{\ifthmt@listswap Example~2.18\else \numberline {2.18}Example\fi }{16}{example.2.18}\protected@file@percent }
\newlabel{ex:KSprim24}{{2.18}{16}{}{example.2.18}{}}
\newlabel{ex:KSprim24@cref}{{[example][18][2]2.18}{[1][16][]16}{}{}{}}
\@writefile{loe}{\contentsline {remark}{\ifthmt@listswap Remark~2.19\else \numberline {2.19}Remark\fi }{16}{remark.2.19}\protected@file@percent }
\newlabel{rmk:DIM:Kast_gauge_eq}{{2.19}{16}{}{remark.2.19}{}}
\newlabel{rmk:DIM:Kast_gauge_eq@cref}{{[remark][19][2]2.19}{[1][16][]16}{}{}{}}
\newlabel{sec:backgr:cyc}{{2.4}{16}{Cyclic symmetry and duality}{subsection.2.4}{}}
\newlabel{sec:backgr:cyc@cref}{{[subsection][4][2]2.4}{[1][16][]16}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\tocsubsection {}{2.4}{Cyclic symmetry and duality}}{16}{subsection.2.4}\protected@file@percent }
\newlabel{eq:Shift_dfn}{{2.15}{16}{Cyclic symmetry and duality}{equation.2.15}{}}
\newlabel{eq:Shift_dfn@cref}{{[equation][15][2]2.15}{[1][16][]16}{}{}{}}
\newlabel{eq:cshift_eps_dfn}{{2.16}{16}{Cyclic symmetry and duality}{equation.2.16}{}}
\newlabel{eq:cshift_eps_dfn@cref}{{[equation][16][2]2.16}{[1][16][]16}{}{}{}}
\citation{KLRR}
\citation{KLRR}
\@writefile{lof}{\contentsline {figure}{\numberline {6}{\ignorespaces  Local moves on planar bipartite graphs.}}{17}{figure.caption.10}\protected@file@percent }
\newlabel{fig:moves}{{6}{17}{Local moves on planar bipartite graphs}{figure.caption.10}{}}
\newlabel{fig:moves@cref}{{[figure][6][]6}{[1][17][]17}{}{}{}}
\newlabel{eq:altp_vs_fhat}{{2.17}{17}{Cyclic symmetry and duality}{equation.2.17}{}}
\newlabel{eq:altp_vs_fhat@cref}{{[equation][17][2]2.17}{[1][17][]17}{}{}{}}
\newlabel{eq:altp_Delta}{{2.18}{17}{Cyclic symmetry and duality}{equation.2.18}{}}
\newlabel{eq:altp_Delta@cref}{{[equation][18][2]2.18}{[1][17][]17}{}{}{}}
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~2.20\else \numberline {2.20}Lemma\fi }{17}{lemma.2.20}\protected@file@percent }
\newlabel{lemma:wind_alt}{{2.20}{17}{}{lemma.2.20}{}}
\newlabel{lemma:wind_alt@cref}{{[lemma][20][2]2.20}{[1][17][]17}{}{}{}}
\newlabel{eq:wind_alt}{{2.19}{17}{}{equation.2.19}{}}
\newlabel{eq:wind_alt@cref}{{[equation][19][2]2.19}{[1][17][]17}{}{}{}}
\newlabel{sec:backgr:moves}{{2.5}{17}{Moves on planar bipartite graphs}{subsection.2.5}{}}
\newlabel{sec:backgr:moves@cref}{{[subsection][5][2]2.5}{[1][17][]17}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\tocsubsection {}{2.5}{Moves on planar bipartite graphs}}{17}{subsection.2.5}\protected@file@percent }
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~2.21\else \numberline {2.21}Definition\fi \thmtformatoptarg {Degree-$2$ vertex insertion and removal}}{17}{definition.2.21}\protected@file@percent }
\newlabel{dfn:backgr:moves:contr_uncontr}{{2.21}{17}{Degree-$2$ vertex insertion and removal}{definition.2.21}{}}
\newlabel{dfn:backgr:moves:contr_uncontr@cref}{{[definition][21][2]2.21}{[1][17][]17}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~2.22\else \numberline {2.22}Definition\fi \thmtformatoptarg {Boundary edge insertion/contraction}}{17}{definition.2.22}\protected@file@percent }
\newlabel{dfn:moves:boundary_edge}{{2.22}{17}{Boundary edge insertion/contraction}{definition.2.22}{}}
\newlabel{dfn:moves:boundary_edge@cref}{{[definition][22][2]2.22}{[1][17][]17}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~2.23\else \numberline {2.23}Definition\fi \thmtformatoptarg {Parallel edge reduction}}{17}{definition.2.23}\protected@file@percent }
\newlabel{dfn:DIM:R1}{{2.23}{17}{Parallel edge reduction}{definition.2.23}{}}
\newlabel{dfn:DIM:R1@cref}{{[definition][23][2]2.23}{[1][17][]17}{}{}{}}
\citation{DFLP}
\@writefile{toc}{\contentsline {section}{\tocsection {}{3}{Momentum amplituhedron}}{18}{section.3}\protected@file@percent }
\newlabel{sec:mom}{{3}{18}{Momentum amplituhedron}{section.3}{}}
\newlabel{sec:mom@cref}{{[section][3][]3}{[1][17][]18}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\tocsubsection {}{3.1}{Properties of the momentum amplituhedron map}}{18}{subsection.3.1}\protected@file@percent }
\newlabel{eq:lak_latk}{{3.1}{18}{Properties of the momentum amplituhedron map}{equation.3.1}{}}
\newlabel{eq:lak_latk@cref}{{[equation][1][3]3.1}{[1][18][]18}{}{}{}}
\newlabel{eq:lak_latk2}{{3.2}{18}{Properties of the momentum amplituhedron map}{equation.3.2}{}}
\newlabel{eq:lak_latk2@cref}{{[equation][2][3]3.2}{[1][18][]18}{}{}{}}
\@writefile{loe}{\contentsline {proposition}{\ifthmt@listswap Proposition~3.1\else \numberline {3.1}Proposition\fi \thmtformatoptarg {\cite  [Section~2.2]{DFLP}}}{18}{proposition.3.1}\protected@file@percent }
\newlabel{prop:momLL_basic}{{3.1}{18}{\cite [Section~2.2]{DFLP}}{proposition.3.1}{}}
\newlabel{prop:momLL_basic@cref}{{[proposition][1][3]3.1}{[1][18][]18}{}{}{}}
\newlabel{mom1}{{{{(1)}}}{18}{\cite [Section~2.2]{DFLP}}{Item.15}{}}
\newlabel{mom1@cref}{{[enumi][1][]{{(1)}}}{[1][18][]18}{}{}{}}
\newlabel{mom2}{{{{(2)}}}{18}{\cite [Section~2.2]{DFLP}}{Item.16}{}}
\newlabel{mom2@cref}{{[enumi][2][]{{(2)}}}{[1][18][]18}{}{}{}}
\newlabel{mom3}{{{{(3)}}}{18}{\cite [Section~2.2]{DFLP}}{Item.17}{}}
\newlabel{mom3@cref}{{[enumi][3][]{{(3)}}}{[1][18][]18}{}{}{}}
\newlabel{mom4}{{{{(4)}}}{18}{\cite [Section~2.2]{DFLP}}{Item.18}{}}
\newlabel{mom4@cref}{{[enumi][4][]{{(4)}}}{[1][18][]18}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\tocsubsection {}{3.2}{Extending $(\lambda ,\tilde  \lambda )$ to $(\Lambda ,\tilde  \Lambda )$}}{18}{subsection.3.2}\protected@file@percent }
\@writefile{loe}{\contentsline {proposition}{\ifthmt@listswap Proposition~3.2\else \numberline {3.2}Proposition\fi }{18}{proposition.3.2}\protected@file@percent }
\newlabel{prop:from_la_to_La}{{3.2}{18}{}{proposition.3.2}{}}
\newlabel{prop:from_la_to_La@cref}{{[proposition][2][3]3.2}{[1][18][]18}{}{}{}}
\citation{GKL1}
\citation{Karp}
\@writefile{lof}{\contentsline {figure}{\numberline {7}{\ignorespaces The column vectors of $\lambda '$ (left) and the corresponding solutions to $h(x)=\nu _i$ (right); see the proof of \cref  {prop:from_la_to_La}.}}{19}{figure.caption.11}\protected@file@percent }
\newlabel{fig:Cheb}{{7}{19}{The column vectors of $\la '$ (left) and the corresponding solutions to $h(x)=\slp _i$ (right); see the proof of \cref {prop:from_la_to_La}}{figure.caption.11}{}}
\newlabel{fig:Cheb@cref}{{[figure][7][]7}{[1][18][]19}{}{}{}}
\@writefile{loe}{\contentsline {corollary}{\ifthmt@listswap Corollary~3.3\else \numberline {3.3}Corollary\fi }{19}{corollary.3.3}\protected@file@percent }
\@writefile{loe}{\contentsline {remark}{\ifthmt@listswap Remark~3.4\else \numberline {3.4}Remark\fi }{19}{remark.3.4}\protected@file@percent }
\newlabel{rmk:connected}{{3.4}{19}{}{remark.3.4}{}}
\newlabel{rmk:connected@cref}{{[remark][4][3]3.4}{[1][19][]19}{}{}{}}
\newlabel{sec:cs_mom_ampl}{{3.3}{19}{The cyclically symmetric momentum amplituhedron}{subsection.3.3}{}}
\newlabel{sec:cs_mom_ampl@cref}{{[subsection][3][3]3.3}{[1][19][]19}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\tocsubsection {}{3.3}{The cyclically symmetric momentum amplituhedron}}{19}{subsection.3.3}\protected@file@percent }
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~3.5\else \numberline {3.5}Definition\fi }{19}{definition.3.5}\protected@file@percent }
\citation{GKL1}
\citation{GKL1}
\citation{AHCC}
\citation{abcgpt}
\citation{abcgpt}
\newlabel{eq:lacs_latcs_regangle}{{3.3}{20}{The cyclically symmetric momentum amplituhedron}{equation.3.3}{}}
\newlabel{eq:lacs_latcs_regangle@cref}{{[equation][3][3]3.3}{[1][20][]20}{}{}{}}
\@writefile{loe}{\contentsline {proposition}{\ifthmt@listswap Proposition~3.6\else \numberline {3.6}Proposition\fi }{20}{proposition.3.6}\protected@file@percent }
\newlabel{ssec:MOM:magic_Qla_mom_ampl}{{3.4}{20}{The magic projector \texorpdfstring {$\Qla $}{Q\_lambda}}{subsection.3.4}{}}
\newlabel{ssec:MOM:magic_Qla_mom_ampl@cref}{{[subsection][4][3]3.4}{[1][20][]20}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\tocsubsection {}{3.4}{The magic projector $Q_{\lambda }$}}{20}{subsection.3.4}\protected@file@percent }
\newlabel{eq:intro:Qla}{{3.4}{20}{The magic projector \texorpdfstring {$\Qla $}{Q\_lambda}}{equation.3.4}{}}
\newlabel{eq:intro:Qla@cref}{{[equation][4][3]3.4}{[1][20][]20}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~3.7\else \numberline {3.7}Definition\fi }{20}{definition.3.7}\protected@file@percent }
\newlabel{dfn:TREE:Qlapp}{{3.7}{20}{}{definition.3.7}{}}
\newlabel{dfn:TREE:Qlapp@cref}{{[definition][7][3]3.7}{[1][20][]20}{}{}{}}
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~3.8\else \numberline {3.8}Lemma\fi }{20}{lemma.3.8}\protected@file@percent }
\newlabel{lemma:TREE:magic_homeo}{{3.8}{20}{}{lemma.3.8}{}}
\newlabel{lemma:TREE:magic_homeo@cref}{{[lemma][8][3]3.8}{[1][20][]20}{}{}{}}
\citation{abcgpt}
\citation{LPW}
\citation{LPW}
\citation{abcgpt}
\citation{abcgpt}
\citation{Rietsch_alg}
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~3.9\else \numberline {3.9}Lemma\fi }{21}{lemma.3.9}\protected@file@percent }
\newlabel{lemma:Qlapp_duality}{{3.9}{21}{}{lemma.3.9}{}}
\newlabel{lemma:Qlapp_duality@cref}{{[lemma][9][3]3.9}{[1][21][]21}{}{}{}}
\newlabel{eq:Qlapp_duality}{{3.5}{21}{}{equation.3.5}{}}
\newlabel{eq:Qlapp_duality@cref}{{[equation][5][3]3.5}{[1][21][]21}{}{}{}}
\newlabel{eq:Qlapp_duality_proof}{{3.6}{21}{The magic projector \texorpdfstring {$\Qla $}{Q\_lambda}}{equation.3.6}{}}
\newlabel{eq:Qlapp_duality_proof@cref}{{[equation][6][3]3.6}{[1][21][]21}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~3.10\else \numberline {3.10}Definition\fi \thmtformatoptarg {T-duality for bounded affine permutations}}{21}{definition.3.10}\protected@file@percent }
\newlabel{dfn:T_dual_perm}{{3.10}{21}{T-duality for bounded affine permutations}{definition.3.10}{}}
\newlabel{dfn:T_dual_perm@cref}{{[definition][10][3]3.10}{[1][21][]21}{}{}{}}
\newlabel{eq:fdd_dfn}{{3.7}{21}{T-duality for bounded affine permutations}{equation.3.7}{}}
\newlabel{eq:fdd_dfn@cref}{{[equation][7][3]3.7}{[1][21][]21}{}{}{}}
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~3.11\else \numberline {3.11}Lemma\fi \thmtformatoptarg {\cite  [Lemma~5.8]{LPW}}}{21}{lemma.3.11}\protected@file@percent }
\newlabel{lemma:la_vs_Bounda_Boundb}{{3.11}{21}{\cite [Lemma~5.8]{LPW}}{lemma.3.11}{}}
\newlabel{lemma:la_vs_Bounda_Boundb@cref}{{[lemma][11][3]3.11}{[1][21][]21}{}{}{}}
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~3.12\else \numberline {3.12}Lemma\fi \thmtformatoptarg {\cite  [Equation~(8.25)]{abcgpt}}}{21}{lemma.3.12}\protected@file@percent }
\newlabel{lemma:Qla_Pio}{{3.12}{21}{\cite [Equation~(8.25)]{abcgpt}}{lemma.3.12}{}}
\newlabel{lemma:Qla_Pio@cref}{{[lemma][12][3]3.12}{[1][21][]21}{}{}{}}
\newlabel{eq:gr_neck_minors_C_vs_Chat_Qla}{{3.8}{21}{The magic projector \texorpdfstring {$\Qla $}{Q\_lambda}}{equation.3.8}{}}
\newlabel{eq:gr_neck_minors_C_vs_Chat_Qla@cref}{{[equation][8][3]3.8}{[1][21][]21}{}{}{}}
\@writefile{loe}{\contentsline {proposition}{\ifthmt@listswap Proposition~3.13\else \numberline {3.13}Proposition\fi }{21}{proposition.3.13}\protected@file@percent }
\newlabel{prop:Qla_Ptp}{{3.13}{21}{}{proposition.3.13}{}}
\newlabel{prop:Qla_Ptp@cref}{{[proposition][13][3]3.13}{[1][21][]21}{}{}{}}
\citation{Kenyon_Sheffield}
\citation{Kenyon_Sheffield}
\citation{Lovasz_Plummer}
\@writefile{loe}{\contentsline {corollary}{\ifthmt@listswap Corollary~3.14\else \numberline {3.14}Corollary\fi }{22}{corollary.3.14}\protected@file@percent }
\newlabel{prop:magic_homeo}{{3.14}{22}{}{corollary.3.14}{}}
\newlabel{prop:magic_homeo@cref}{{[corollary][14][3]3.14}{[1][22][]22}{}{}{}}
\@writefile{toc}{\contentsline {section}{\tocsection {}{4}{Dimer formulae for Kenyon--Smirnov primitives\xspace  }}{22}{section.4}\protected@file@percent }
\newlabel{sec:dimer_KS}{{4}{22}{Dimer formulae for \KSprims }{section.4}{}}
\newlabel{sec:dimer_KS@cref}{{[section][4][]4}{[1][22][]22}{}{}{}}
\newlabel{ssec:surplus}{{4.1}{22}{Surplus}{subsection.4.1}{}}
\newlabel{ssec:surplus@cref}{{[subsection][1][4]4.1}{[1][22][]22}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\tocsubsection {}{4.1}{Surplus}}{22}{subsection.4.1}\protected@file@percent }
\@writefile{loe}{\contentsline {proposition}{\ifthmt@listswap Proposition~4.1\else \numberline {4.1}Proposition\fi }{22}{proposition.4.1}\protected@file@percent }
\newlabel{prop:DIM:helWBmin_geq_0=>apm_exists}{{4.1}{22}{}{proposition.4.1}{}}
\newlabel{prop:DIM:helWBmin_geq_0=>apm_exists@cref}{{[proposition][1][4]4.1}{[1][22][]22}{}{}{}}
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~4.2\else \numberline {4.2}Lemma\fi }{22}{lemma.4.2}\protected@file@percent }
\newlabel{lemma:DIM:deleting_hel_verts}{{4.2}{22}{}{lemma.4.2}{}}
\newlabel{lemma:DIM:deleting_hel_verts@cref}{{[lemma][2][4]4.2}{[1][22][]22}{}{}{}}
\newlabel{DIM:del1}{{{{(1)}}}{22}{}{Item.19}{}}
\newlabel{DIM:del1@cref}{{[enumi][1][]{{(1)}}}{[1][22][]22}{}{}{}}
\newlabel{DIM:del2}{{{{(2)}}}{22}{}{Item.20}{}}
\newlabel{DIM:del2@cref}{{[enumi][2][]{{(2)}}}{[1][22][]22}{}{}{}}
\@writefile{loe}{\contentsline {corollary}{\ifthmt@listswap Corollary~4.3\else \numberline {4.3}Corollary\fi }{22}{corollary.4.3}\protected@file@percent }
\newlabel{lemma:hel_geq_1}{{4.3}{22}{}{corollary.4.3}{}}
\newlabel{lemma:hel_geq_1@cref}{{[corollary][3][4]4.3}{[1][22][]22}{}{}{}}
\citation{origami2}
\citation{origami2}
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~4.4\else \numberline {4.4}Lemma\fi }{23}{lemma.4.4}\protected@file@percent }
\newlabel{lemma:DIM:moves_vs_helWmin_trivalent}{{4.4}{23}{}{lemma.4.4}{}}
\newlabel{lemma:DIM:moves_vs_helWmin_trivalent@cref}{{[lemma][4][4]4.4}{[1][23][]23}{}{}{}}
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~4.5\else \numberline {4.5}Lemma\fi }{23}{lemma.4.5}\protected@file@percent }
\newlabel{lemma:DIM:moves_vs_helWmin}{{4.5}{23}{}{lemma.4.5}{}}
\newlabel{lemma:DIM:moves_vs_helWmin@cref}{{[lemma][5][4]4.5}{[1][23][]23}{}{}{}}
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~4.6\else \numberline {4.6}Lemma\fi }{23}{lemma.4.6}\protected@file@percent }
\newlabel{lemma:reduced_helmin}{{4.6}{23}{}{lemma.4.6}{}}
\newlabel{lemma:reduced_helmin@cref}{{[lemma][6][4]4.6}{[1][23][]23}{}{}{}}
\newlabel{reduced_helmin1}{{{{(1)}}}{23}{}{Item.21}{}}
\newlabel{reduced_helmin1@cref}{{[enumi][1][]{{(1)}}}{[1][23][]23}{}{}{}}
\newlabel{reduced_helmin2}{{{{(2)}}}{23}{}{Item.22}{}}
\newlabel{reduced_helmin2@cref}{{[enumi][2][]{{(2)}}}{[1][23][]23}{}{}{}}
\@writefile{loe}{\contentsline {remark}{\ifthmt@listswap Remark~4.7\else \numberline {4.7}Remark\fi }{23}{remark.4.7}\protected@file@percent }
\newlabel{rmk:reduced_helmin2}{{4.7}{23}{}{remark.4.7}{}}
\newlabel{rmk:reduced_helmin2@cref}{{[remark][7][4]4.7}{[1][23][]23}{}{}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {8}{\ignorespaces  A path $\gamma $ and the corresponding zig-zag cut $\xi _{\gamma }$ (left); the zig-zag cuts $\xi _i,\xi _j$ in the proof of \cref  {lemma:TE:single_dimer_formula} (middle); tripod insertion (right). }}{24}{figure.caption.12}\protected@file@percent }
\newlabel{fig:zig-cut}{{8}{24}{A path $\Path $ and the corresponding zig-zag cut $\CutP $ (left); the zig-zag cuts $\Cut _i,\Cut _j$ in the proof of \cref {lemma:TE:single_dimer_formula} (middle); tripod insertion (right)}{figure.caption.12}{}}
\newlabel{fig:zig-cut@cref}{{[figure][8][]8}{[1][24][]24}{}{}{}}
\newlabel{ssec:TE:Kast}{{4.2}{24}{Type $(2,4)$: single-dimer configurations}{subsection.4.2}{}}
\newlabel{ssec:TE:Kast@cref}{{[subsection][2][4]4.2}{[1][23][]24}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\tocsubsection {}{4.2}{Type $(2,4)$: single-dimer configurations}}{24}{subsection.4.2}\protected@file@percent }
\newlabel{eq:TE:y_to_lalat}{{4.1}{24}{Type $(2,4)$: single-dimer configurations}{equation.4.1}{}}
\newlabel{eq:TE:y_to_lalat@cref}{{[equation][1][4]4.1}{[1][24][]24}{}{}{}}
\@writefile{loe}{\contentsline {proposition}{\ifthmt@listswap Proposition~4.8\else \numberline {4.8}Proposition\fi }{24}{proposition.4.8}\protected@file@percent }
\newlabel{lemma:TE:single_dimer_formula}{{4.8}{24}{}{proposition.4.8}{}}
\newlabel{lemma:TE:single_dimer_formula@cref}{{[proposition][8][4]4.8}{[1][24][]24}{}{}{}}
\newlabel{eq:IP:brlaw}{{4.2}{24}{}{equation.4.2}{}}
\newlabel{eq:IP:brlaw@cref}{{[equation][2][4]4.2}{[1][24][]24}{}{}{}}
\newlabel{eq:IP:brlatb}{{4.3}{24}{}{equation.4.3}{}}
\newlabel{eq:IP:brlatb@cref}{{[equation][3][4]4.3}{[1][24][]24}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~4.9\else \numberline {4.9}Definition\fi \thmtformatoptarg {Tripod insertion}}{24}{definition.4.9}\protected@file@percent }
\newlabel{dfn:eksbb}{{4.9}{24}{Tripod insertion}{definition.4.9}{}}
\newlabel{dfn:eksbb@cref}{{[definition][9][4]4.9}{[1][24][]24}{}{}{}}
\@writefile{loe}{\contentsline {remark}{\ifthmt@listswap Remark~4.10\else \numberline {4.10}Remark\fi }{25}{remark.4.10}\protected@file@percent }
\newlabel{rmk:tripods_commute}{{4.10}{25}{}{remark.4.10}{}}
\newlabel{rmk:tripods_commute@cref}{{[remark][10][4]4.10}{[1][25][]25}{}{}{}}
\newlabel{eq:TE:constw=constb=1}{{4.4}{26}{Type $(2,4)$: single-dimer configurations}{equation.4.4}{}}
\newlabel{eq:TE:constw=constb=1@cref}{{[equation][4][4]4.4}{[1][26][]26}{}{}{}}
\@writefile{loe}{\contentsline {corollary}{\ifthmt@listswap Corollary~4.11\else \numberline {4.11}Corollary\fi }{26}{corollary.4.11}\protected@file@percent }
\newlabel{lemma:TE:single_dimer_same_face}{{4.11}{26}{}{corollary.4.11}{}}
\newlabel{lemma:TE:single_dimer_same_face@cref}{{[corollary][11][4]4.11}{[1][26][]26}{}{}{}}
\newlabel{eq:TE:same_face}{{4.5}{26}{}{equation.4.5}{}}
\newlabel{eq:TE:same_face@cref}{{[equation][5][4]4.5}{[1][26][]26}{}{}{}}
\newlabel{eq:*}{{4.6}{26}{Type $(2,4)$: single-dimer configurations}{equation.4.6}{}}
\newlabel{eq:*@cref}{{[equation][6][4]4.6}{[1][26][]26}{}{}{}}
\newlabel{ssec:TE:Kast2}{{4.3}{26}{Type $(2,4)$: double-dimer configurations}{subsection.4.3}{}}
\newlabel{ssec:TE:Kast2@cref}{{[subsection][3][4]4.3}{[1][26][]26}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\tocsubsection {}{4.3}{Type $(2,4)$: double-dimer configurations}}{26}{subsection.4.3}\protected@file@percent }
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~4.12\else \numberline {4.12}Definition\fi }{26}{definition.4.12}\protected@file@percent }
\newlabel{dfn:double_dimer_Omf}{{4.12}{26}{}{definition.4.12}{}}
\newlabel{dfn:double_dimer_Omf@cref}{{[definition][12][4]4.12}{[1][26][]26}{}{}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {9}{\ignorespaces  Computing $\varepsilon _{\text  {\scalebox {0.85}{$\mathtt  {alt}$}}}(\setbox \z@ \hbox {\mathsurround \z@ $\textstyle \Omega $}\mathaccent "0365{\Omega }^{\bullet \to \circ }_{e_1,e_2})$; see \cref  {lemma:TE:Omvec,lemma:TE:OmsGf_pos}.}}{27}{figure.caption.13}\protected@file@percent }
\newlabel{fig:eps-alt}{{9}{27}{Computing $\epsOmf (\Omfvecbw _{\e _1,\e _2})$; see \cref {lemma:TE:Omvec,lemma:TE:OmsGf_pos}}{figure.caption.13}{}}
\newlabel{fig:eps-alt@cref}{{[figure][9][]9}{[1][27][]27}{}{}{}}
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~4.13\else \numberline {4.13}Lemma\fi }{27}{lemma.4.13}\protected@file@percent }
\newlabel{lemma:TE:Omvec}{{4.13}{27}{}{lemma.4.13}{}}
\newlabel{lemma:TE:Omvec@cref}{{[lemma][13][4]4.13}{[1][27][]27}{}{}{}}
\newlabel{eq:TE:Omvec}{{4.7}{27}{}{equation.4.7}{}}
\newlabel{eq:TE:Omvec@cref}{{[equation][7][4]4.7}{[1][27][]27}{}{}{}}
\@writefile{loe}{\contentsline {proposition}{\ifthmt@listswap Proposition~4.14\else \numberline {4.14}Proposition\fi }{28}{proposition.4.14}\protected@file@percent }
\newlabel{lemma:TE:OmsGf_pos}{{4.14}{28}{}{proposition.4.14}{}}
\newlabel{lemma:TE:OmsGf_pos@cref}{{[proposition][14][4]4.14}{[1][27][]28}{}{}{}}
\newlabel{eq:TE:OmsGf_pos}{{4.8}{28}{}{equation.4.8}{}}
\newlabel{eq:TE:OmsGf_pos@cref}{{[equation][8][4]4.8}{[1][28][]28}{}{}{}}
\newlabel{eq:TE:Mand_RHS_proof}{{4.9}{28}{Type $(2,4)$: double-dimer configurations}{equation.4.9}{}}
\newlabel{eq:TE:Mand_RHS_proof@cref}{{[equation][9][4]4.9}{[1][28][]28}{}{}{}}
\newlabel{ssec:annular}{{4.4}{28}{Annular graphs and momentum amplituhedron map}{subsection.4.4}{}}
\newlabel{ssec:annular@cref}{{[subsection][4][4]4.4}{[1][28][]28}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\tocsubsection {}{4.4}{Annular graphs and momentum amplituhedron map}}{28}{subsection.4.4}\protected@file@percent }
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~4.15\else \numberline {4.15}Definition\fi }{28}{definition.4.15}\protected@file@percent }
\newlabel{eq:OAC:Cbotpm_meas}{{4.10}{29}{Annular graphs and momentum amplituhedron map}{equation.4.10}{}}
\newlabel{eq:OAC:Cbotpm_meas@cref}{{[equation][10][4]4.10}{[1][28][]29}{}{}{}}
\@writefile{loe}{\contentsline {remark}{\ifthmt@listswap Remark~4.16\else \numberline {4.16}Remark\fi }{29}{remark.4.16}\protected@file@percent }
\newlabel{rmk:OAC:turn_Gbot_into_sphere}{{4.16}{29}{}{remark.4.16}{}}
\newlabel{rmk:OAC:turn_Gbot_into_sphere@cref}{{[remark][16][4]4.16}{[1][29][]29}{}{}{}}
\newlabel{eq:OCA:Cbotm_subset_Cbotp}{{4.11}{29}{}{equation.4.11}{}}
\newlabel{eq:OCA:Cbotm_subset_Cbotp@cref}{{[equation][11][4]4.11}{[1][29][]29}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~4.17\else \numberline {4.17}Definition\fi }{29}{definition.4.17}\protected@file@percent }
\newlabel{dfn:OAC:Arep}{{4.17}{29}{}{definition.4.17}{}}
\newlabel{dfn:OAC:Arep@cref}{{[definition][17][4]4.17}{[1][29][]29}{}{}{}}
\newlabel{eq:OAC:Arep}{{4.12}{29}{}{equation.4.12}{}}
\newlabel{eq:OAC:Arep@cref}{{[equation][12][4]4.12}{[1][29][]29}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~4.18\else \numberline {4.18}Definition\fi \thmtformatoptarg {Gluing planar bipartite graphs}}{29}{definition.4.18}\protected@file@percent }
\newlabel{def:OAC:stacking_graphs}{{4.18}{29}{Gluing planar bipartite graphs}{definition.4.18}{}}
\newlabel{def:OAC:stacking_graphs@cref}{{[definition][18][4]4.18}{[1][29][]29}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~4.19\else \numberline {4.19}Definition\fi }{29}{definition.4.19}\protected@file@percent }
\newlabel{eq:OAC:epsKf_stacked}{{4.13}{29}{Annular graphs and momentum amplituhedron map}{equation.4.13}{}}
\newlabel{eq:OAC:epsKf_stacked@cref}{{[equation][13][4]4.13}{[1][29][]29}{}{}{}}
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~4.20\else \numberline {4.20}Lemma\fi }{29}{lemma.4.20}\protected@file@percent }
\citation{Lus2}
\citation{LamCDM}
\citation{BlKa}
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~4.21\else \numberline {4.21}Lemma\fi }{30}{lemma.4.21}\protected@file@percent }
\newlabel{lemma:OAC:Gf_satisfies_ass}{{4.21}{30}{}{lemma.4.21}{}}
\newlabel{lemma:OAC:Gf_satisfies_ass@cref}{{[lemma][21][4]4.21}{[1][30][]30}{}{}{}}
\@writefile{loe}{\contentsline {corollary}{\ifthmt@listswap Corollary~4.22\else \numberline {4.22}Corollary\fi }{30}{corollary.4.22}\protected@file@percent }
\newlabel{cor:Ann_split_Delta}{{4.22}{30}{}{corollary.4.22}{}}
\newlabel{cor:Ann_split_Delta@cref}{{[corollary][22][4]4.22}{[1][30][]30}{}{}{}}
\newlabel{eq:Ann_split_Deltaw}{{4.14}{30}{}{equation.4.14}{}}
\newlabel{eq:Ann_split_Deltaw@cref}{{[equation][14][4]4.14}{[1][30][]30}{}{}{}}
\newlabel{eq:Ann_split_Deltab}{{4.15}{30}{}{equation.4.15}{}}
\newlabel{eq:Ann_split_Deltab@cref}{{[equation][15][4]4.15}{[1][30][]30}{}{}{}}
\newlabel{ssec:flag_positive}{{4.5}{30}{Flag-positive pairs \texorpdfstring {$(\La ,\Lat )$}{(𝚲,𝚲̃)}}{subsection.4.5}{}}
\newlabel{ssec:flag_positive@cref}{{[subsection][5][4]4.5}{[1][30][]30}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\tocsubsection {}{4.5}{Flag-positive pairs $(\Lambda ,\tilde  \Lambda )$}}{30}{subsection.4.5}\protected@file@percent }
\newlabel{eq:OAC:pifl}{{4.16}{30}{Flag-positive pairs \texorpdfstring {$(\La ,\Lat )$}{(𝚲,𝚲̃)}}{equation.4.16}{}}
\newlabel{eq:OAC:pifl@cref}{{[equation][16][4]4.16}{[1][30][]30}{}{}{}}
\citation{Pos}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~4.23\else \numberline {4.23}Definition\fi }{31}{definition.4.23}\protected@file@percent }
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~4.24\else \numberline {4.24}Lemma\fi }{31}{lemma.4.24}\protected@file@percent }
\newlabel{lemma:OAC:flag_pos=>Arep}{{4.24}{31}{}{lemma.4.24}{}}
\newlabel{lemma:OAC:flag_pos=>Arep@cref}{{[lemma][24][4]4.24}{[1][31][]31}{}{}{}}
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~4.25\else \numberline {4.25}Lemma\fi }{31}{lemma.4.25}\protected@file@percent }
\newlabel{lemma:OAC:stacking_vs_PhiLL}{{4.25}{31}{}{lemma.4.25}{}}
\newlabel{lemma:OAC:stacking_vs_PhiLL@cref}{{[lemma][25][4]4.25}{[1][31][]31}{}{}{}}
\@writefile{loe}{\contentsline {corollary}{\ifthmt@listswap Corollary~4.26\else \numberline {4.26}Corollary\fi }{31}{corollary.4.26}\protected@file@percent }
\newlabel{cor:lak_implies_black_imm}{{4.26}{31}{}{corollary.4.26}{}}
\newlabel{cor:lak_implies_black_imm@cref}{{[corollary][26][4]4.26}{[1][31][]31}{}{}{}}
\newlabel{lak_implies1}{{{{(1)}}}{31}{}{Item.23}{}}
\newlabel{lak_implies1@cref}{{[enumi][1][]{{(1)}}}{[1][31][]31}{}{}{}}
\newlabel{lak_implies2}{{{{(2)}}}{31}{}{Item.24}{}}
\newlabel{lak_implies2@cref}{{[enumi][2][]{{(2)}}}{[1][31][]31}{}{}{}}
\newlabel{lak_implies3}{{{{(3)}}}{31}{}{Item.25}{}}
\newlabel{lak_implies3@cref}{{[enumi][3][]{{(3)}}}{[1][31][]31}{}{}{}}
\newlabel{eq:TE:same_face_and_same_vertex}{{4.17}{31}{}{equation.4.17}{}}
\newlabel{eq:TE:same_face_and_same_vertex@cref}{{[equation][17][4]4.17}{[1][31][]31}{}{}{}}
\newlabel{lak_implies4}{{{{(4)}}}{31}{}{Item.26}{}}
\newlabel{lak_implies4@cref}{{[enumi][4][]{{(4)}}}{[1][31][]31}{}{}{}}
\@writefile{loe}{\contentsline {corollary}{\ifthmt@listswap Corollary~4.27\else \numberline {4.27}Corollary\fi }{32}{corollary.4.27}\protected@file@percent }
\newlabel{eq:IP:brlaw_G}{{4.18}{32}{}{equation.4.18}{}}
\newlabel{eq:IP:brlaw_G@cref}{{[equation][18][4]4.18}{[1][32][]32}{}{}{}}
\newlabel{eq:IP:brlatb_G}{{4.19}{32}{}{equation.4.19}{}}
\newlabel{eq:IP:brlatb_G@cref}{{[equation][19][4]4.19}{[1][32][]32}{}{}{}}
\@writefile{loe}{\contentsline {remark}{\ifthmt@listswap Remark~4.28\else \numberline {4.28}Remark\fi }{32}{remark.4.28}\protected@file@percent }
\newlabel{rmk:can_add_edges}{{4.28}{32}{}{remark.4.28}{}}
\newlabel{rmk:can_add_edges@cref}{{[remark][28][4]4.28}{[1][32][]32}{}{}{}}
\@writefile{toc}{\contentsline {section}{\tocsection {}{5}{Proof of origami-amplituhedron correspondence\xspace  }}{32}{section.5}\protected@file@percent }
\newlabel{sec:proof_main_bij}{{5}{32}{Proof of \oac }{section.5}{}}
\newlabel{sec:proof_main_bij@cref}{{[section][5][]5}{[1][32][]32}{}{}{}}
\newlabel{sec:proof_main:from_t_imm_to_triples}{{5.1}{32}{From t-immersions to triples of subspaces}{subsection.5.1}{}}
\newlabel{sec:proof_main:from_t_imm_to_triples@cref}{{[subsection][1][5]5.1}{[1][32][]32}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\tocsubsection {}{5.1}{From t-immersions to triples of subspaces}}{32}{subsection.5.1}\protected@file@percent }
\citation{KLRR}
\citation{CLR1}
\citation{KLRR}
\citation{CLR1}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~5.1\else \numberline {5.1}Definition\fi }{33}{definition.5.1}\protected@file@percent }
\newlabel{dfn:TE:datr}{{5.1}{33}{}{definition.5.1}{}}
\newlabel{dfn:TE:datr@cref}{{[definition][1][5]5.1}{[1][32][]33}{}{}{}}
\@writefile{loe}{\contentsline {proposition}{\ifthmt@listswap Proposition~5.2\else \numberline {5.2}Proposition\fi \thmtformatoptarg {\cite  [Section~3.2]{KLRR} and \cite  [Sections~2 and~3]{CLR1}}}{33}{proposition.5.2}\protected@file@percent }
\newlabel{prop:t_imm=>holom}{{5.2}{33}{\cite [Section~3.2]{KLRR} and \cite [Sections~2 and~3]{CLR1}}{proposition.5.2}{}}
\newlabel{prop:t_imm=>holom@cref}{{[proposition][2][5]5.2}{[1][33][]33}{}{}{}}
\@writefile{loe}{\contentsline {remark}{\ifthmt@listswap Remark~5.3\else \numberline {5.3}Remark\fi }{33}{remark.5.3}\protected@file@percent }
\newlabel{rmk:Fw_Fb_determined_up_to_const}{{5.3}{33}{}{remark.5.3}{}}
\newlabel{rmk:Fw_Fb_determined_up_to_const@cref}{{[remark][3][5]5.3}{[1][33][]33}{}{}{}}
\@writefile{loe}{\contentsline {proposition}{\ifthmt@listswap Proposition~5.4\else \numberline {5.4}Proposition\fi }{33}{proposition.5.4}\protected@file@percent }
\newlabel{prop:t_imm=>TRIPLES}{{5.4}{33}{}{proposition.5.4}{}}
\newlabel{prop:t_imm=>TRIPLES@cref}{{[proposition][4][5]5.4}{[1][33][]33}{}{}{}}
\newlabel{eq:yy=Tcal_Ocal}{{5.1}{33}{From t-immersions to triples of subspaces}{equation.5.1}{}}
\newlabel{eq:yy=Tcal_Ocal@cref}{{[equation][1][5]5.1}{[1][33][]33}{}{}{}}
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~5.5\else \numberline {5.5}Lemma\fi }{33}{lemma.5.5}\protected@file@percent }
\newlabel{lemma:angle_sum_arg_rat}{{5.5}{33}{}{lemma.5.5}{}}
\newlabel{lemma:angle_sum_arg_rat@cref}{{[lemma][5][5]5.5}{[1][33][]33}{}{}{}}
\newlabel{eq:angle_sum_arg_rat}{{5.2}{33}{}{equation.5.2}{}}
\newlabel{eq:angle_sum_arg_rat@cref}{{[equation][2][5]5.2}{[1][33][]33}{}{}{}}
\newlabel{eq:T_Kast_bdry}{{5.3}{34}{From t-immersions to triples of subspaces}{equation.5.3}{}}
\newlabel{eq:T_Kast_bdry@cref}{{[equation][3][5]5.3}{[1][34][]34}{}{}{}}
\@writefile{loe}{\contentsline {corollary}{\ifthmt@listswap Corollary~5.6\else \numberline {5.6}Corollary\fi }{34}{corollary.5.6}\protected@file@percent }
\newlabel{cor:t_imm_=>_<ii+1>>0}{{5.6}{34}{}{corollary.5.6}{}}
\newlabel{cor:t_imm_=>_<ii+1>>0@cref}{{[corollary][6][5]5.6}{[1][34][]34}{}{}{}}
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~5.7\else \numberline {5.7}Lemma\fi }{34}{lemma.5.7}\protected@file@percent }
\newlabel{eq:sumw_sumb_pi_k}{{5.4}{34}{}{equation.5.4}{}}
\newlabel{eq:sumw_sumb_pi_k@cref}{{[equation][4][5]5.4}{[1][34][]34}{}{}{}}
\newlabel{eq:sum_up_angles1}{{5.5}{34}{From t-immersions to triples of subspaces}{equation.5.5}{}}
\newlabel{eq:sum_up_angles1@cref}{{[equation][5][5]5.5}{[1][34][]34}{}{}{}}
\newlabel{eq:sum_up_angles2}{{5.6}{34}{From t-immersions to triples of subspaces}{equation.5.6}{}}
\newlabel{eq:sum_up_angles2@cref}{{[equation][6][5]5.6}{[1][34][]34}{}{}{}}
\newlabel{sec:finishing_main_bij}{{5.2}{34}{From triples of subspaces to t-immersions}{subsection.5.2}{}}
\newlabel{sec:finishing_main_bij@cref}{{[subsection][2][5]5.2}{[1][34][]34}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\tocsubsection {}{5.2}{From triples of subspaces to t-immersions}}{34}{thmt@dummyctr.dummy.93}\protected@file@percent }
\@writefile{loe}{\contentsline {notation}{\ifthmt@listswap Notation~5.8\else \numberline {5.8}Notation\fi }{34}{notation.5.8}\protected@file@percent }
\newlabel{notn:Tll_xll}{{5.8}{34}{}{notation.5.8}{}}
\newlabel{notn:Tll_xll@cref}{{[notation][8][5]5.8}{[1][34][]34}{}{}{}}
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~5.9\else \numberline {5.9}Lemma\fi }{34}{lemma.5.9}\protected@file@percent }
\newlabel{lemma:OAC:nondeg}{{5.9}{34}{}{lemma.5.9}{}}
\newlabel{lemma:OAC:nondeg@cref}{{[lemma][9][5]5.9}{[1][34][]34}{}{}{}}
\@writefile{loe}{\contentsline {proposition}{\ifthmt@listswap Proposition~5.10\else \numberline {5.10}Proposition\fi }{35}{proposition.5.10}\protected@file@percent }
\newlabel{lemma:Tll_is_t_imm}{{5.10}{35}{}{proposition.5.10}{}}
\newlabel{lemma:Tll_is_t_imm@cref}{{[proposition][10][5]5.10}{[1][35][]35}{}{}{}}
\newlabel{eq:angle_ineqs_inside}{{5.7}{35}{From triples of subspaces to t-immersions}{equation.5.7}{}}
\newlabel{eq:angle_ineqs_inside@cref}{{[equation][7][5]5.7}{[1][35][]35}{}{}{}}
\newlabel{eq:angle_ineqs_bdry}{{5.8}{35}{From triples of subspaces to t-immersions}{equation.5.8}{}}
\newlabel{eq:angle_ineqs_bdry@cref}{{[equation][8][5]5.8}{[1][35][]35}{}{}{}}
\citation{RhSk}
\citation{Lam_dimers}
\citation{Lam_dimers}
\@writefile{toc}{\contentsline {section}{\tocsection {}{6}{Mandelstam variables, immanants, and t-embeddings}}{36}{section.6}\protected@file@percent }
\newlabel{sec:imm}{{6}{36}{Mandelstam variables, immanants, and t-embeddings}{section.6}{}}
\newlabel{sec:imm@cref}{{[section][6][]6}{[1][36][]36}{}{}{}}
\newlabel{sec:TL_imm}{{6.1}{36}{Temperley--Lieb immanants}{subsection.6.1}{}}
\newlabel{sec:TL_imm@cref}{{[subsection][1][6]6.1}{[1][36][]36}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\tocsubsection {}{6.1}{Temperley--Lieb immanants}}{36}{subsection.6.1}\protected@file@percent }
\newlabel{eq:TL_imm_dfn}{{6.1}{36}{Temperley--Lieb immanants}{equation.6.1}{}}
\newlabel{eq:TL_imm_dfn@cref}{{[equation][1][6]6.1}{[1][36][]36}{}{}{}}
\newlabel{eq:Delta_tauT_vs_OmsGtauT}{{6.2}{36}{Temperley--Lieb immanants}{equation.6.2}{}}
\newlabel{eq:Delta_tauT_vs_OmsGtauT@cref}{{[equation][2][6]6.2}{[1][36][]36}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\tocsubsection {}{6.2}{Immanants of $(\Lambda ,\tilde  \Lambda )$}}{36}{subsection.6.2}\protected@file@percent }
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~6.1\else \numberline {6.1}Definition\fi \thmtformatoptarg {Markings}}{36}{definition.6.1}\protected@file@percent }
\newlabel{dfn:markings_Om}{{6.1}{36}{Markings}{definition.6.1}{}}
\newlabel{dfn:markings_Om@cref}{{[definition][1][6]6.1}{[1][36][]36}{}{}{}}
\newlabel{marking1}{{{{(1)}}}{36}{Markings}{Item.27}{}}
\newlabel{marking1@cref}{{[enumi][1][]{{(1)}}}{[1][36][]36}{}{}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {10}{\ignorespaces  Two $(\Omega ,f^\ast ,g^\ast )$-markings (see \cref  {dfn:markings_Om}). The elements in $T_{\Omega }$ (resp., $\bm  {[n]}\setminus (T_{\Omega }\sqcup S(\tau _{\Omega }))$) are marked by $\textcolor {blue}{\operatorname  {T}}$ (resp., $\textcolor {blue}{\emptyset }$). The paths $\gamma ^\partial _1,\gamma ^\partial _2$ are shown in blue. }}{37}{figure.caption.14}\protected@file@percent }
\newlabel{fig:marking}{{10}{37}{Two $\Omfg $-markings (see \cref {dfn:markings_Om}). The elements in $\TOm $ (resp., $\brn \setminus (\TOm \sqcup \StauOm )$) are marked by $\textcolor {blue}{\Tmark }$ (resp., $\textcolor {blue}{\Emark }$). The paths $\Pathbd _1,\Pathbd _2$ are shown in blue}{figure.caption.14}{}}
\newlabel{fig:marking@cref}{{[figure][10][]10}{[1][36][]37}{}{}{}}
\@writefile{loe}{\contentsline {proposition}{\ifthmt@listswap Proposition~6.2\else \numberline {6.2}Proposition\fi }{37}{proposition.6.2}\protected@file@percent }
\newlabel{lemma:immanant_fg}{{6.2}{37}{}{proposition.6.2}{}}
\newlabel{lemma:immanant_fg@cref}{{[proposition][2][6]6.2}{[1][37][]37}{}{}{}}
\newlabel{eq:immanant_fg}{{6.3}{37}{}{equation.6.3}{}}
\newlabel{eq:immanant_fg@cref}{{[equation][3][6]6.3}{[1][37][]37}{}{}{}}
\newlabel{eq:immanant_fg_dfn}{{6.4}{37}{}{equation.6.4}{}}
\newlabel{eq:immanant_fg_dfn@cref}{{[equation][4][6]6.4}{[1][37][]37}{}{}{}}
\newlabel{eq:TE:Omvec_G}{{6.5}{37}{Immanants of \texorpdfstring {$(\La ,\Lat )$}{(𝚲,𝚲̃)}}{equation.6.5}{}}
\newlabel{eq:TE:Omvec_G@cref}{{[equation][5][6]6.5}{[1][37][]37}{}{}{}}
\newlabel{eq:TE:Omvec_G_TtaucoefOmee}{{6.6}{37}{Immanants of \texorpdfstring {$(\La ,\Lat )$}{(𝚲,𝚲̃)}}{equation.6.6}{}}
\newlabel{eq:TE:Omvec_G_TtaucoefOmee@cref}{{[equation][6][6]6.6}{[1][37][]37}{}{}{}}
\citation{DFLP}
\citation{Parisi_thesis}
\@writefile{lof}{\contentsline {figure}{\numberline {11}{\ignorespaces  A matching $\tau $ and the six $(\tau ,T,i,j)$-markings; see \cref  {ex:tau_markings}.}}{38}{figure.caption.15}\protected@file@percent }
\newlabel{fig:tau}{{11}{38}{A matching $\tau $ and the six $\Ttauij $-markings; see \cref {ex:tau_markings}}{figure.caption.15}{}}
\newlabel{fig:tau@cref}{{[figure][11][]11}{[1][38][]38}{}{}{}}
\@writefile{loe}{\contentsline {corollary}{\ifthmt@listswap Corollary~6.3\else \numberline {6.3}Corollary\fi }{38}{corollary.6.3}\protected@file@percent }
\newlabel{thm:Mand_Ttau}{{6.3}{38}{}{corollary.6.3}{}}
\newlabel{thm:Mand_Ttau@cref}{{[corollary][3][6]6.3}{[1][38][]38}{}{}{}}
\newlabel{eq:Mand_Ttau}{{6.7}{38}{}{equation.6.7}{}}
\newlabel{eq:Mand_Ttau@cref}{{[equation][7][6]6.7}{[1][38][]38}{}{}{}}
\@writefile{loe}{\contentsline {example}{\ifthmt@listswap Example~6.4\else \numberline {6.4}Example\fi }{38}{example.6.4}\protected@file@percent }
\newlabel{ex:tau_markings}{{6.4}{38}{}{example.6.4}{}}
\newlabel{ex:tau_markings@cref}{{[example][4][6]6.4}{[1][38][]38}{}{}{}}
\newlabel{eq:intro:imm_example}{{6.8}{38}{}{equation.6.8}{}}
\newlabel{eq:intro:imm_example@cref}{{[equation][8][6]6.8}{[1][38][]38}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~6.5\else \numberline {6.5}Definition\fi \thmtformatoptarg {Immanants of $(\Lambda ,\tilde  \Lambda )$}}{38}{definition.6.5}\protected@file@percent }
\newlabel{dfn:immanants_LaLat}{{6.5}{38}{Immanants of $\LaLat $}{definition.6.5}{}}
\newlabel{dfn:immanants_LaLat@cref}{{[definition][5][6]6.5}{[1][38][]38}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~6.6\else \numberline {6.6}Definition\fi }{38}{definition.6.6}\protected@file@percent }
\newlabel{dfn:Ttauknij}{{6.6}{38}{}{definition.6.6}{}}
\newlabel{dfn:Ttauknij@cref}{{[definition][6][6]6.6}{[1][38][]38}{}{}{}}
\@writefile{loe}{\contentsline {remark}{\ifthmt@listswap Remark~6.7\else \numberline {6.7}Remark\fi }{38}{remark.6.7}\protected@file@percent }
\newlabel{rmk:Ttauknij_>0_vs_0}{{6.7}{38}{}{remark.6.7}{}}
\newlabel{rmk:Ttauknij_>0_vs_0@cref}{{[remark][7][6]6.7}{[1][38][]38}{}{}{}}
\@writefile{loe}{\contentsline {remark}{\ifthmt@listswap Remark~6.8\else \numberline {6.8}Remark\fi }{39}{remark.6.8}\protected@file@percent }
\newlabel{eq:Ttaucoef_fg_vs_ij}{{6.9}{39}{}{equation.6.9}{}}
\newlabel{eq:Ttaucoef_fg_vs_ij@cref}{{[equation][9][6]6.9}{[1][39][]39}{}{}{}}
\newlabel{ssec:annular_immanants}{{6.3}{39}{Immanants of annular graphs}{subsection.6.3}{}}
\newlabel{ssec:annular_immanants@cref}{{[subsection][3][6]6.3}{[1][39][]39}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\tocsubsection {}{6.3}{Immanants of annular graphs}}{39}{subsection.6.3}\protected@file@percent }
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~6.9\else \numberline {6.9}Definition\fi }{39}{definition.6.9}\protected@file@percent }
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~6.10\else \numberline {6.10}Definition\fi }{39}{definition.6.10}\protected@file@percent }
\@writefile{loe}{\contentsline {corollary}{\ifthmt@listswap Corollary~6.11\else \numberline {6.11}Corollary\fi }{39}{corollary.6.11}\protected@file@percent }
\newlabel{eq:OmsGf_vs_Ttaucoef}{{6.10}{39}{}{equation.6.10}{}}
\newlabel{eq:OmsGf_vs_Ttaucoef@cref}{{[equation][10][6]6.10}{[1][39][]39}{}{}{}}
\@writefile{loe}{\contentsline {example}{\ifthmt@listswap Example~6.12\else \numberline {6.12}Example\fi }{39}{example.6.12}\protected@file@percent }
\newlabel{ex:Arep-not-immp}{{6.12}{39}{}{example.6.12}{}}
\newlabel{ex:Arep-not-immp@cref}{{[example][12][6]6.12}{[1][39][]39}{}{}{}}
\citation{Lam_dimers}
\@writefile{lof}{\contentsline {figure}{\numberline {12}{\ignorespaces  The graph $\breve  {\Gamma }$ gives rise to an $\breve  {\mathbb  {A}}$-representable\xspace  pair $(\Lambda ,\tilde  \Lambda )$ which is immanant-nonnegative but not immanant-positive; see \cref  {ex:Arep-not-immp}. }}{40}{figure.caption.16}\protected@file@percent }
\newlabel{fig:Arep-not-immp}{{12}{40}{The graph $\Gbot $ gives rise to an \Arep pair $\LaLat $ which is immanant-nonnegative but not immanant-positive; see \cref {ex:Arep-not-immp}}{figure.caption.16}{}}
\newlabel{fig:Arep-not-immp@cref}{{[figure][12][]12}{[1][39][]40}{}{}{}}
\@writefile{loe}{\contentsline {proposition}{\ifthmt@listswap Proposition~6.13\else \numberline {6.13}Proposition\fi }{40}{proposition.6.13}\protected@file@percent }
\newlabel{lemma:Arep_subset_immnn}{{6.13}{40}{}{proposition.6.13}{}}
\newlabel{lemma:Arep_subset_immnn@cref}{{[proposition][13][6]6.13}{[1][39][]40}{}{}{}}
\newlabel{eq:Ttaucoef(LaLat)=Ttaucoef(Gbot,wtbot)}{{6.11}{40}{}{equation.6.11}{}}
\newlabel{eq:Ttaucoef(LaLat)=Ttaucoef(Gbot,wtbot)@cref}{{[equation][11][6]6.11}{[1][39][]40}{}{}{}}
\newlabel{eq:Mand_vs_OmsGf}{{6.12}{40}{Immanants of annular graphs}{equation.6.12}{}}
\newlabel{eq:Mand_vs_OmsGf@cref}{{[equation][12][6]6.12}{[1][40][]40}{}{}{}}
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~6.14\else \numberline {6.14}Lemma\fi }{40}{lemma.6.14}\protected@file@percent }
\newlabel{lemma:Ttaucoef_nonzero_on_Fl}{{6.14}{40}{}{lemma.6.14}{}}
\newlabel{lemma:Ttaucoef_nonzero_on_Fl@cref}{{[lemma][14][6]6.14}{[1][40][]40}{}{}{}}
\@writefile{loe}{\contentsline {corollary}{\ifthmt@listswap Corollary~6.15\else \numberline {6.15}Corollary\fi }{40}{corollary.6.15}\protected@file@percent }
\newlabel{thm:imm_pos_Fltp}{{6.15}{40}{}{corollary.6.15}{}}
\newlabel{thm:imm_pos_Fltp@cref}{{[corollary][15][6]6.15}{[1][40][]40}{}{}{}}
\citation{Lam_dimers}
\citation{DFLP}
\@writefile{loe}{\contentsline {corollary}{\ifthmt@listswap Corollary~6.16\else \numberline {6.16}Corollary\fi }{41}{corollary.6.16}\protected@file@percent }
\newlabel{lemma:LaLaimmp_nonempty_Z_dense}{{6.16}{41}{}{corollary.6.16}{}}
\newlabel{lemma:LaLaimmp_nonempty_Z_dense@cref}{{[corollary][16][6]6.16}{[1][41][]41}{}{}{}}
\@writefile{loe}{\contentsline {remark}{\ifthmt@listswap Remark~6.17\else \numberline {6.17}Remark\fi }{41}{remark.6.17}\protected@file@percent }
\newlabel{eq:inclusions_LaLa}{{6.13}{41}{Immanants of annular graphs}{equation.6.13}{}}
\newlabel{eq:inclusions_LaLa@cref}{{[equation][13][6]6.13}{[1][41][]41}{}{}{}}
\@writefile{loe}{\contentsline {question}{\ifthmt@listswap Question~6.18\else \numberline {6.18}Question\fi }{41}{question.6.18}\protected@file@percent }
\newlabel{que:immp_vs_flag_vs_Arep}{{6.18}{41}{}{question.6.18}{}}
\newlabel{que:immp_vs_flag_vs_Arep@cref}{{[question][18][6]6.18}{[1][41][]41}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\tocsubsection {}{6.4}{$2$-separated\xspace  faces}}{41}{thmt@dummyctr.dummy.114}\protected@file@percent }
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~6.19\else \numberline {6.19}Definition\fi }{41}{definition.6.19}\protected@file@percent }
\newlabel{dfn:PROP:2sep}{{6.19}{41}{}{definition.6.19}{}}
\newlabel{dfn:PROP:2sep@cref}{{[definition][19][6]6.19}{[1][41][]41}{}{}{}}
\@writefile{loe}{\contentsline {remark}{\ifthmt@listswap Remark~6.20\else \numberline {6.20}Remark\fi }{41}{remark.6.20}\protected@file@percent }
\newlabel{rmk:exactly_twosep}{{6.20}{41}{}{remark.6.20}{}}
\newlabel{rmk:exactly_twosep@cref}{{[remark][20][6]6.20}{[1][41][]41}{}{}{}}
\@writefile{loe}{\contentsline {corollary}{\ifthmt@listswap Corollary~6.21\else \numberline {6.21}Corollary\fi }{41}{corollary.6.21}\protected@file@percent }
\newlabel{lemma:PROP:Mpos}{{6.21}{41}{}{corollary.6.21}{}}
\newlabel{lemma:PROP:Mpos@cref}{{[corollary][21][6]6.21}{[1][41][]41}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~6.22\else \numberline {6.22}Definition\fi }{41}{definition.6.22}\protected@file@percent }
\newlabel{dfn:fullysep}{{6.22}{41}{}{definition.6.22}{}}
\newlabel{dfn:fullysep@cref}{{[definition][22][6]6.22}{[1][41][]41}{}{}{}}
\citation{Talaska}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~6.23\else \numberline {6.23}Definition\fi }{42}{definition.6.23}\protected@file@percent }
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~6.24\else \numberline {6.24}Lemma\fi }{42}{lemma.6.24}\protected@file@percent }
\newlabel{lemma:TREE:fullysep_vs_rhoij}{{6.24}{42}{}{lemma.6.24}{}}
\newlabel{lemma:TREE:fullysep_vs_rhoij@cref}{{[lemma][24][6]6.24}{[1][42][]42}{}{}{}}
\newlabel{rho1:twosep}{{{{(1)}}}{42}{}{Item.29}{}}
\newlabel{rho1:twosep@cref}{{[enumi][1][]{{(1)}}}{[1][42][]42}{}{}{}}
\newlabel{rho2:GO}{{{{(2)}}}{42}{}{Item.30}{}}
\newlabel{rho2:GO@cref}{{[enumi][2][]{{(2)}}}{[1][42][]42}{}{}{}}
\newlabel{rho3:rhoij}{{{{(3)}}}{42}{}{Item.31}{}}
\newlabel{rho3:rhoij@cref}{{[enumi][3][]{{(3)}}}{[1][42][]42}{}{}{}}
\newlabel{rho4:share_face}{{{{(4)}}}{42}{}{Item.32}{}}
\newlabel{rho4:share_face@cref}{{[enumi][4][]{{(4)}}}{[1][42][]42}{}{}{}}
\newlabel{eq:rhoij_k_Iij_Iji}{{6.14}{42}{\Twosep faces}{equation.6.14}{}}
\newlabel{eq:rhoij_k_Iij_Iji@cref}{{[equation][14][6]6.14}{[1][42][]42}{}{}{}}
\newlabel{eq:rho_claim}{{6.15}{42}{\Twosep faces}{equation.6.15}{}}
\newlabel{eq:rho_claim@cref}{{[equation][15][6]6.15}{[1][42][]42}{}{}{}}
\@writefile{loe}{\contentsline {corollary}{\ifthmt@listswap Corollary~6.25\else \numberline {6.25}Corollary\fi }{43}{corollary.6.25}\protected@file@percent }
\newlabel{lemma:imm_pos_Mand_pos}{{6.25}{43}{}{corollary.6.25}{}}
\newlabel{lemma:imm_pos_Mand_pos@cref}{{[corollary][25][6]6.25}{[1][43][]43}{}{}{}}
\@writefile{loe}{\contentsline {corollary}{\ifthmt@listswap Corollary~6.26\else \numberline {6.26}Corollary\fi }{43}{corollary.6.26}\protected@file@percent }
\newlabel{lemma:fullysep=>twonondeg}{{6.26}{43}{}{corollary.6.26}{}}
\newlabel{lemma:fullysep=>twonondeg@cref}{{[corollary][26][6]6.26}{[1][43][]43}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~6.27\else \numberline {6.27}Definition\fi }{43}{definition.6.27}\protected@file@percent }
\newlabel{dfn:Grfsep}{{6.27}{43}{}{definition.6.27}{}}
\newlabel{dfn:Grfsep@cref}{{[definition][27][6]6.27}{[1][43][]43}{}{}{}}
\newlabel{eq:Grfsep_dfn}{{6.16}{43}{}{equation.6.16}{}}
\newlabel{eq:Grfsep_dfn@cref}{{[equation][16][6]6.16}{[1][43][]43}{}{}{}}
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~6.28\else \numberline {6.28}Lemma\fi }{43}{lemma.6.28}\protected@file@percent }
\newlabel{lemma:lalat_MP=>C_fsep}{{6.28}{43}{}{lemma.6.28}{}}
\newlabel{lemma:lalat_MP=>C_fsep@cref}{{[lemma][28][6]6.28}{[1][43][]43}{}{}{}}
\citation{Suho_rank}
\citation{Suho_rank}
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~6.29\else \numberline {6.29}Lemma\fi }{44}{lemma.6.29}\protected@file@percent }
\newlabel{lemma:TREE:rank_of_iijj}{{6.29}{44}{}{lemma.6.29}{}}
\newlabel{lemma:TREE:rank_of_iijj@cref}{{[lemma][29][6]6.29}{[1][43][]44}{}{}{}}
\newlabel{eq:TREE:rank_of_iijj}{{6.17}{44}{}{equation.6.17}{}}
\newlabel{eq:TREE:rank_of_iijj@cref}{{[equation][17][6]6.17}{[1][44][]44}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~6.30\else \numberline {6.30}Definition\fi }{44}{definition.6.30}\protected@file@percent }
\newlabel{dfn:Grfind}{{6.30}{44}{}{definition.6.30}{}}
\newlabel{dfn:Grfind@cref}{{[definition][30][6]6.30}{[1][44][]44}{}{}{}}
\newlabel{ssec:Mbd_and_temb}{{6.5}{44}{\MbdTITLE and t-embeddings}{subsection.6.5}{}}
\newlabel{ssec:Mbd_and_temb@cref}{{[subsection][5][6]6.5}{[1][44][]44}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\tocsubsection {}{6.5}{Mandelstam-positive boundary\xspace  and t-embeddings}}{44}{subsection.6.5}\protected@file@percent }
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~6.31\else \numberline {6.31}Definition\fi }{44}{definition.6.31}\protected@file@percent }
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~6.32\else \numberline {6.32}Lemma\fi }{44}{lemma.6.32}\protected@file@percent }
\newlabel{lemma:non_self_intersecting_Sigma}{{6.32}{44}{}{lemma.6.32}{}}
\newlabel{lemma:non_self_intersecting_Sigma@cref}{{[lemma][32][6]6.32}{[1][44][]44}{}{}{}}
\newlabel{bdrysi1}{{{{(i)}}}{44}{\MbdTITLE and t-embeddings}{Item.33}{}}
\newlabel{bdrysi1@cref}{{[enumi][1][]{{(i)}}}{[1][44][]44}{}{}{}}
\newlabel{bdrysi2}{{{{(ii)}}}{44}{\MbdTITLE and t-embeddings}{Item.34}{}}
\newlabel{bdrysi2@cref}{{[enumi][2][]{{(ii)}}}{[1][44][]44}{}{}{}}
\newlabel{bdrysi3}{{{{(iii)}}}{44}{\MbdTITLE and t-embeddings}{Item.35}{}}
\newlabel{bdrysi3@cref}{{[enumi][3][]{{(iii)}}}{[1][44][]44}{}{}{}}
\citation{CLR2}
\@writefile{loe}{\contentsline {remark}{\ifthmt@listswap Remark~6.33\else \numberline {6.33}Remark\fi }{45}{remark.6.33}\protected@file@percent }
\newlabel{rmk:K4}{{6.33}{45}{}{remark.6.33}{}}
\newlabel{rmk:K4@cref}{{[remark][33][6]6.33}{[1][45][]45}{}{}{}}
\@writefile{loe}{\contentsline {corollary}{\ifthmt@listswap Corollary~6.34\else \numberline {6.34}Corollary\fi }{45}{corollary.6.34}\protected@file@percent }
\newlabel{lemma:Mbd=>simple}{{6.34}{45}{}{corollary.6.34}{}}
\newlabel{lemma:Mbd=>simple@cref}{{[corollary][34][6]6.34}{[1][45][]45}{}{}{}}
\@writefile{loe}{\contentsline {corollary}{\ifthmt@listswap Corollary~6.35\else \numberline {6.35}Corollary\fi }{45}{corollary.6.35}\protected@file@percent }
\newlabel{lemma:fullysep=>simple_and_Mbd}{{6.35}{45}{}{corollary.6.35}{}}
\newlabel{lemma:fullysep=>simple_and_Mbd@cref}{{[corollary][35][6]6.35}{[1][45][]45}{}{}{}}
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~6.36\else \numberline {6.36}Lemma\fi }{45}{lemma.6.36}\protected@file@percent }
\newlabel{lemma:helmin>2=>no_triangles}{{6.36}{45}{}{lemma.6.36}{}}
\newlabel{lemma:helmin>2=>no_triangles@cref}{{[lemma][36][6]6.36}{[1][45][]45}{}{}{}}
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~6.37\else \numberline {6.37}Lemma\fi }{45}{lemma.6.37}\protected@file@percent }
\newlabel{lemma:LaLaimmn+helmin=simple}{{6.37}{45}{}{lemma.6.37}{}}
\newlabel{lemma:LaLaimmn+helmin=simple@cref}{{[lemma][37][6]6.37}{[1][45][]45}{}{}{}}
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~6.38\else \numberline {6.38}Lemma\fi }{45}{lemma.6.38}\protected@file@percent }
\newlabel{lemma:Jordan_curve}{{6.38}{45}{}{lemma.6.38}{}}
\newlabel{lemma:Jordan_curve@cref}{{[lemma][38][6]6.38}{[1][45][]45}{}{}{}}
\@writefile{loe}{\contentsline {corollary}{\ifthmt@listswap Corollary~6.39\else \numberline {6.39}Corollary\fi }{46}{corollary.6.39}\protected@file@percent }
\newlabel{lemma:LaLaimmn+helmin=t_emb}{{6.39}{46}{}{corollary.6.39}{}}
\newlabel{lemma:LaLaimmn+helmin=t_emb@cref}{{[corollary][39][6]6.39}{[1][46][]46}{}{}{}}
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~6.40\else \numberline {6.40}Lemma\fi }{46}{lemma.6.40}\protected@file@percent }
\newlabel{lemma:weakMbd=>boundary>0_or_=0}{{6.40}{46}{}{lemma.6.40}{}}
\newlabel{lemma:weakMbd=>boundary>0_or_=0@cref}{{[lemma][40][6]6.40}{[1][46][]46}{}{}{}}
\@writefile{loe}{\contentsline {proposition}{\ifthmt@listswap Proposition~6.41\else \numberline {6.41}Proposition\fi }{46}{proposition.6.41}\protected@file@percent }
\newlabel{lemma:Mbd=>face_Mnn}{{6.41}{46}{}{proposition.6.41}{}}
\newlabel{lemma:Mbd=>face_Mnn@cref}{{[proposition][41][6]6.41}{[1][46][]46}{}{}{}}
\citation{abcgpt}
\citation{KWZ}
\citation{abcgpt}
\citation{KWZ}
\@writefile{toc}{\contentsline {section}{\tocsection {}{7}{BCFW tilings of ambient momentum amplituhedra}}{47}{section.7}\protected@file@percent }
\newlabel{sec:BCFW}{{7}{47}{BCFW tilings of ambient momentum amplituhedra}{section.7}{}}
\newlabel{sec:BCFW@cref}{{[section][7][]7}{[1][47][]47}{}{}{}}
\newlabel{sec:BCFW:backgr}{{7.1}{47}{Background on the BCFW recursion}{subsection.7.1}{}}
\newlabel{sec:BCFW:backgr@cref}{{[subsection][1][7]7.1}{[1][47][]47}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\tocsubsection {}{7.1}{Background on the BCFW recursion}}{47}{subsection.7.1}\protected@file@percent }
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~7.1\else \numberline {7.1}Definition\fi \thmtformatoptarg {BCFW recursion}}{47}{definition.7.1}\protected@file@percent }
\newlabel{dfn:BCFW}{{7.1}{47}{BCFW recursion}{definition.7.1}{}}
\newlabel{dfn:BCFW@cref}{{[definition][1][7]7.1}{[1][47][]47}{}{}{}}
\newlabel{step_BCFW1}{{{{(1)}}}{47}{BCFW recursion}{Item.36}{}}
\newlabel{step_BCFW1@cref}{{[enumi][1][]{{(1)}}}{[1][47][]47}{}{}{}}
\newlabel{step_BCFW2}{{{{(2)}}}{47}{BCFW recursion}{Item.37}{}}
\newlabel{step_BCFW2@cref}{{[enumi][2][]{{(2)}}}{[1][47][]47}{}{}{}}
\newlabel{BCFW1}{{{{(BCFW1)}}}{47}{BCFW recursion}{Item.38}{}}
\newlabel{BCFW1@cref}{{[enumii][1][2]{{(BCFW1)}}}{[1][47][]47}{}{}{}}
\newlabel{BCFW2}{{{{(BCFW2)}}}{47}{BCFW recursion}{Item.39}{}}
\newlabel{BCFW2@cref}{{[enumii][2][2]{{(BCFW2)}}}{[1][47][]47}{}{}{}}
\newlabel{BCFW3}{{{{(BCFW3)}}}{47}{BCFW recursion}{Item.40}{}}
\newlabel{BCFW3@cref}{{[enumii][3][2]{{(BCFW3)}}}{[1][47][]47}{}{}{}}
\@writefile{loe}{\contentsline {remark}{\ifthmt@listswap Remark~7.2\else \numberline {7.2}Remark\fi }{47}{remark.7.2}\protected@file@percent }
\newlabel{rmk:jo}{{7.2}{47}{}{remark.7.2}{}}
\newlabel{rmk:jo@cref}{{[remark][2][7]7.2}{[1][47][]47}{}{}{}}
\@writefile{loe}{\contentsline {remark}{\ifthmt@listswap Remark~7.3\else \numberline {7.3}Remark\fi }{47}{remark.7.3}\protected@file@percent }
\newlabel{rmk:BCFW_multiple}{{7.3}{47}{}{remark.7.3}{}}
\newlabel{rmk:BCFW_multiple@cref}{{[remark][3][7]7.3}{[1][47][]47}{}{}{}}
\@writefile{loe}{\contentsline {remark}{\ifthmt@listswap Remark~7.4\else \numberline {7.4}Remark\fi }{47}{remark.7.4}\protected@file@percent }
\newlabel{rmk:BCFW_reduced}{{7.4}{47}{}{remark.7.4}{}}
\newlabel{rmk:BCFW_reduced@cref}{{[remark][4][7]7.4}{[1][47][]47}{}{}{}}
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~7.5\else \numberline {7.5}Lemma\fi }{47}{lemma.7.5}\protected@file@percent }
\newlabel{lemma:BCFW_fullysep}{{7.5}{47}{}{lemma.7.5}{}}
\newlabel{lemma:BCFW_fullysep@cref}{{[lemma][5][7]7.5}{[1][47][]47}{}{}{}}
\citation{ABL}
\citation{ABL}
\@writefile{loe}{\contentsline {corollary}{\ifthmt@listswap Corollary~7.6\else \numberline {7.6}Corollary\fi }{48}{corollary.7.6}\protected@file@percent }
\newlabel{cor:BCFW:share_face}{{7.6}{48}{}{corollary.7.6}{}}
\newlabel{cor:BCFW:share_face@cref}{{[corollary][6][7]7.6}{[1][47][]48}{}{}{}}
\newlabel{sec:BCFW:triangulation_MP}{{7.2}{48}{BCFW tilings}{subsection.7.2}{}}
\newlabel{sec:BCFW:triangulation_MP@cref}{{[subsection][2][7]7.2}{[1][48][]48}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\tocsubsection {}{7.2}{BCFW tilings}}{48}{subsection.7.2}\protected@file@percent }
\newlabel{eq:lalappf_dfn}{{7.1}{48}{BCFW tilings}{equation.7.1}{}}
\newlabel{eq:lalappf_dfn@cref}{{[equation][1][7]7.1}{[1][48][]48}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~7.7\else \numberline {7.7}Definition\fi \thmtformatoptarg {$\mathcal  {R}$-Tiling\xspace  }}{48}{definition.7.7}\protected@file@percent }
\newlabel{dfn:BCFW:tiling_amb}{{7.7}{48}{\Mtiling }{definition.7.7}{}}
\newlabel{dfn:BCFW:tiling_amb@cref}{{[definition][7][7]7.7}{[1][48][]48}{}{}{}}
\newlabel{eq:BCFW:tile_amb_dfn}{{7.2}{48}{\Mtiling }{equation.7.2}{}}
\newlabel{eq:BCFW:tile_amb_dfn@cref}{{[equation][2][7]7.2}{[1][48][]48}{}{}{}}
\newlabel{Rtiling1}{{{{(a)}}}{48}{\Mtiling }{Item.41}{}}
\newlabel{Rtiling1@cref}{{[enumi][1][]{{(a)}}}{[1][48][]48}{}{}{}}
\newlabel{Rtiling2}{{{{(b)}}}{48}{\Mtiling }{Item.42}{}}
\newlabel{Rtiling2@cref}{{[enumi][2][]{{(b)}}}{[1][48][]48}{}{}{}}
\newlabel{Rtiling3}{{{{(c)}}}{48}{\Mtiling }{Item.43}{}}
\newlabel{Rtiling3@cref}{{[enumi][3][]{{(c)}}}{[1][48][]48}{}{}{}}
\newlabel{eq:TREE:Rel_dfn}{{7.3}{48}{BCFW tilings}{equation.7.3}{}}
\newlabel{eq:TREE:Rel_dfn@cref}{{[equation][3][7]7.3}{[1][48][]48}{}{}{}}
\@writefile{loe}{\contentsline {theorem}{\ifthmt@listswap Theorem~7.8\else \numberline {7.8}Theorem\fi \thmtformatoptarg {BCFW tilings of ambient momentum amplituhedra}}{48}{theorem.7.8}\protected@file@percent }
\newlabel{thm:f_triang}{{7.8}{48}{BCFW tilings of ambient momentum amplituhedra}{theorem.7.8}{}}
\newlabel{thm:f_triang@cref}{{[theorem][8][7]7.8}{[1][48][]48}{}{}{}}
\@writefile{loe}{\contentsline {remark}{\ifthmt@listswap Remark~7.9\else \numberline {7.9}Remark\fi }{48}{remark.7.9}\protected@file@percent }
\newlabel{rmk:BCFW:T_emb_unique}{{7.9}{48}{}{remark.7.9}{}}
\newlabel{rmk:BCFW:T_emb_unique@cref}{{[remark][9][7]7.9}{[1][48][]48}{}{}{}}
\newlabel{eq:lalaC_ppf}{{7.4}{48}{}{equation.7.4}{}}
\newlabel{eq:lalaC_ppf@cref}{{[equation][4][7]7.4}{[1][48][]48}{}{}{}}
\@writefile{loe}{\contentsline {remark}{\ifthmt@listswap Remark~7.10\else \numberline {7.10}Remark\fi }{48}{remark.7.10}\protected@file@percent }
\newlabel{rmk:dim_MomLL2}{{7.10}{48}{}{remark.7.10}{}}
\newlabel{rmk:dim_MomLL2@cref}{{[remark][10][7]7.10}{[1][48][]48}{}{}{}}
\@writefile{loe}{\contentsline {remark}{\ifthmt@listswap Remark~7.11\else \numberline {7.11}Remark\fi \thmtformatoptarg {Ambient momentum amplituhedron canonical form}}{48}{remark.7.11}\protected@file@percent }
\newlabel{rmk:omega_form}{{7.11}{48}{Ambient momentum amplituhedron canonical form}{remark.7.11}{}}
\newlabel{rmk:omega_form@cref}{{[remark][11][7]7.11}{[1][48][]48}{}{}{}}
\citation{ElHu}
\newlabel{sec:particle_momenta}{{7.3}{49}{Particle momenta and Mandelstam variables}{subsection.7.3}{}}
\newlabel{sec:particle_momenta@cref}{{[subsection][3][7]7.3}{[1][49][]49}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\tocsubsection {}{7.3}{Particle momenta and Mandelstam variables}}{49}{subsection.7.3}\protected@file@percent }
\newlabel{eq:Pmom_cdot_Qmom}{{7.5}{49}{Particle momenta and Mandelstam variables}{equation.7.5}{}}
\newlabel{eq:Pmom_cdot_Qmom@cref}{{[equation][5][7]7.5}{[1][49][]49}{}{}{}}
\newlabel{eq:Pmom_vs_yyt}{{7.6}{49}{Particle momenta and Mandelstam variables}{equation.7.6}{}}
\newlabel{eq:Pmom_vs_yyt@cref}{{[equation][6][7]7.6}{[1][49][]49}{}{}{}}
\newlabel{eq:Pmom_Qmom_det}{{7.7}{49}{Particle momenta and Mandelstam variables}{equation.7.7}{}}
\newlabel{eq:Pmom_Qmom_det@cref}{{[equation][7][7]7.7}{[1][49][]49}{}{}{}}
\newlabel{eq:bispinor_cdot}{{7.8}{49}{Particle momenta and Mandelstam variables}{equation.7.8}{}}
\newlabel{eq:bispinor_cdot@cref}{{[equation][8][7]7.8}{[1][49][]49}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~7.12\else \numberline {7.12}Definition\fi }{49}{definition.7.12}\protected@file@percent }
\newlabel{dfn:Pll}{{7.12}{49}{}{definition.7.12}{}}
\newlabel{dfn:Pll@cref}{{[definition][12][7]7.12}{[1][49][]49}{}{}{}}
\newlabel{eq:Pmom_scalar}{{7.9}{49}{Particle momenta and Mandelstam variables}{equation.7.9}{}}
\newlabel{eq:Pmom_scalar@cref}{{[equation][9][7]7.9}{[1][49][]49}{}{}{}}
\newlabel{eq:Mand_vs_norm_proof}{{7.10}{49}{Particle momenta and Mandelstam variables}{equation.7.10}{}}
\newlabel{eq:Mand_vs_norm_proof@cref}{{[equation][10][7]7.10}{[1][49][]49}{}{}{}}
\@writefile{loe}{\contentsline {remark}{\ifthmt@listswap Remark~7.13\else \numberline {7.13}Remark\fi \thmtformatoptarg {Inversion}}{49}{remark.7.13}\protected@file@percent }
\newlabel{rmk:dual_conformal}{{7.13}{49}{Inversion}{remark.7.13}{}}
\newlabel{rmk:dual_conformal@cref}{{[remark][13][7]7.13}{[1][49][]49}{}{}{}}
\citation{CheRa}
\citation{CLR1}
\citation{CLR2}
\citation{AlMa}
\@writefile{loe}{\contentsline {remark}{\ifthmt@listswap Remark~7.14\else \numberline {7.14}Remark\fi }{50}{remark.7.14}\protected@file@percent }
\newlabel{sec:BCFW:boundary}{{7.4}{50}{Boundary data}{subsection.7.4}{}}
\newlabel{sec:BCFW:boundary@cref}{{[subsection][4][7]7.4}{[1][50][]50}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\tocsubsection {}{7.4}{Boundary data}}{50}{subsection.7.4}\protected@file@percent }
\@writefile{loe}{\contentsline {remark}{\ifthmt@listswap Remark~7.15\else \numberline {7.15}Remark\fi }{50}{remark.7.15}\protected@file@percent }
\newlabel{rmk:bdry:alpha}{{7.15}{50}{}{remark.7.15}{}}
\newlabel{rmk:bdry:alpha@cref}{{[remark][15][7]7.15}{[1][50][]50}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~7.16\else \numberline {7.16}Definition\fi }{50}{definition.7.16}\protected@file@percent }
\newlabel{dfn:BCFW:little_group}{{7.16}{50}{}{definition.7.16}{}}
\newlabel{dfn:BCFW:little_group@cref}{{[definition][16][7]7.16}{[1][50][]50}{}{}{}}
\@writefile{loe}{\contentsline {remark}{\ifthmt@listswap Remark~7.17\else \numberline {7.17}Remark\fi }{50}{remark.7.17}\protected@file@percent }
\newlabel{rmk:BCFW:little_group}{{7.17}{50}{}{remark.7.17}{}}
\newlabel{rmk:BCFW:little_group@cref}{{[remark][17][7]7.17}{[1][50][]50}{}{}{}}
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~7.18\else \numberline {7.18}Lemma\fi }{50}{lemma.7.18}\protected@file@percent }
\newlabel{lemma:BCFW:null}{{7.18}{50}{}{lemma.7.18}{}}
\newlabel{lemma:BCFW:null@cref}{{[lemma][18][7]7.18}{[1][50][]50}{}{}{}}
\newlabel{eq:sum_arg_pmom_-2pi}{{7.11}{50}{}{equation.7.11}{}}
\newlabel{eq:sum_arg_pmom_-2pi@cref}{{[equation][11][7]7.11}{[1][50][]50}{}{}{}}
\@writefile{loe}{\contentsline {remark}{\ifthmt@listswap Remark~7.19\else \numberline {7.19}Remark\fi }{50}{remark.7.19}\protected@file@percent }
\newlabel{rmk:arg_Pmom_ratio}{{7.19}{50}{}{remark.7.19}{}}
\newlabel{rmk:arg_Pmom_ratio@cref}{{[remark][19][7]7.19}{[1][50][]50}{}{}{}}
\citation{BCFW}
\citation{ElHu}
\newlabel{eq:BCFW:sumwP_sumbP_dfn}{{7.12}{51}{}{equation.7.12}{}}
\newlabel{eq:BCFW:sumwP_sumbP_dfn@cref}{{[equation][12][7]7.12}{[1][50][]51}{}{}{}}
\newlabel{eq:wind_Pcurve_vs_wind_lalat}{{7.13}{51}{}{equation.7.13}{}}
\newlabel{eq:wind_Pcurve_vs_wind_lalat@cref}{{[equation][13][7]7.13}{[1][51][]51}{}{}{}}
\@writefile{loe}{\contentsline {remark}{\ifthmt@listswap Remark~7.20\else \numberline {7.20}Remark\fi }{51}{remark.7.20}\protected@file@percent }
\newlabel{rmk:BCFW:null_triangle}{{7.20}{51}{}{remark.7.20}{}}
\newlabel{rmk:BCFW:null_triangle@cref}{{[remark][20][7]7.20}{[1][51][]51}{}{}{}}
\newlabel{ssec:BCFW_boundary}{{7.5}{51}{BCFW boundary data}{subsection.7.5}{}}
\newlabel{ssec:BCFW_boundary@cref}{{[subsection][5][7]7.5}{[1][51][]51}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\tocsubsection {}{7.5}{BCFW boundary data}}{51}{subsection.7.5}\protected@file@percent }
\newlabel{eq:Rmom_dfn}{{7.14}{51}{BCFW boundary data}{equation.7.14}{}}
\newlabel{eq:Rmom_dfn@cref}{{[equation][14][7]7.14}{[1][51][]51}{}{}{}}
\newlabel{eq:Psum_r_dfn}{{7.15}{51}{BCFW boundary data}{equation.7.15}{}}
\newlabel{eq:Psum_r_dfn@cref}{{[equation][15][7]7.15}{[1][51][]51}{}{}{}}
\@writefile{loe}{\contentsline {remark}{\ifthmt@listswap Remark~7.21\else \numberline {7.21}Remark\fi }{51}{remark.7.21}\protected@file@percent }
\newlabel{rmk:coincides_BCFW}{{7.21}{51}{}{remark.7.21}{}}
\newlabel{rmk:coincides_BCFW@cref}{{[remark][21][7]7.21}{[1][51][]51}{}{}{}}
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~7.22\else \numberline {7.22}Lemma\fi }{51}{lemma.7.22}\protected@file@percent }
\newlabel{lemma:bisector}{{7.22}{51}{}{lemma.7.22}{}}
\newlabel{lemma:bisector@cref}{{[lemma][22][7]7.22}{[1][51][]51}{}{}{}}
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~7.23\else \numberline {7.23}Lemma\fi }{51}{lemma.7.23}\protected@file@percent }
\newlabel{lemma:BCFW:rs_not_in_interval}{{7.23}{51}{}{lemma.7.23}{}}
\newlabel{lemma:BCFW:rs_not_in_interval@cref}{{[lemma][23][7]7.23}{[1][51][]51}{}{}{}}
\newlabel{sec:BCFW:proof_a_b}{{7.6}{51}{T-embeddings of BCFW graphs}{subsection.7.6}{}}
\newlabel{sec:BCFW:proof_a_b@cref}{{[subsection][6][7]7.6}{[1][51][]51}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\tocsubsection {}{7.6}{T-embeddings of BCFW graphs}}{51}{subsection.7.6}\protected@file@percent }
\@writefile{loe}{\contentsline {proposition}{\ifthmt@listswap Proposition~7.24\else \numberline {7.24}Proposition\fi }{52}{proposition.7.24}\protected@file@percent }
\newlabel{prop:BCFW:from_lalat_to_r}{{7.24}{52}{}{proposition.7.24}{}}
\newlabel{prop:BCFW:from_lalat_to_r@cref}{{[proposition][24][7]7.24}{[1][52][]52}{}{}{}}
\newlabel{sec:BCFW:from_lalat_to_t_emb}{{7.7}{52}{\ORATITLE }{subsection.7.7}{}}
\newlabel{sec:BCFW:from_lalat_to_t_emb@cref}{{[subsection][7][7]7.7}{[1][52][]52}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\tocsubsection {}{7.7}{Origami reconstruction algorithm\xspace  }}{52}{subsection.7.7}\protected@file@percent }
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~7.25\else \numberline {7.25}Lemma\fi }{52}{lemma.7.25}\protected@file@percent }
\newlabel{lemma:ray_inside_polygon}{{7.25}{52}{}{lemma.7.25}{}}
\newlabel{lemma:ray_inside_polygon@cref}{{[lemma][25][7]7.25}{[1][52][]52}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~7.26\else \numberline {7.26}Definition\fi }{53}{definition.7.26}\protected@file@percent }
\newlabel{dfn:BCFW:generic}{{7.26}{53}{}{definition.7.26}{}}
\newlabel{dfn:BCFW:generic@cref}{{[definition][26][7]7.26}{[1][53][]53}{}{}{}}
\@writefile{loe}{\contentsline {corollary}{\ifthmt@listswap Corollary~7.27\else \numberline {7.27}Corollary\fi }{53}{corollary.7.27}\protected@file@percent }
\newlabel{cor:BCFW:Mand_pos}{{7.27}{53}{}{corollary.7.27}{}}
\newlabel{cor:BCFW:Mand_pos@cref}{{[corollary][27][7]7.27}{[1][53][]53}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~7.28\else \numberline {7.28}Definition\fi }{53}{definition.7.28}\protected@file@percent }
\newlabel{dfn:msgen}{{7.28}{53}{}{definition.7.28}{}}
\newlabel{dfn:msgen@cref}{{[definition][28][7]7.28}{[1][53][]53}{}{}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {13}{\ignorespaces  The null polygons ${\bm  {a}}_L,{\bm  {a}}_R,{\bm  {b}}_L,{\bm  {b}}_R,{\bm  {c}}_L,{\bm  {c}}_R$ projected to the kami plane.}}{54}{figure.caption.17}\protected@file@percent }
\newlabel{fig:ABC}{{13}{54}{The null polygons $\AcurveL ,\AcurveR ,\BcurveL ,\BcurveR ,\CcurveL ,\CcurveR $ projected to the kami plane}{figure.caption.17}{}}
\newlabel{fig:ABC@cref}{{[figure][13][]13}{[1][54][]54}{}{}{}}
\@writefile{loe}{\contentsline {remark}{\ifthmt@listswap Remark~7.29\else \numberline {7.29}Remark\fi }{54}{remark.7.29}\protected@file@percent }
\newlabel{rmk:msgen}{{7.29}{54}{}{remark.7.29}{}}
\newlabel{rmk:msgen@cref}{{[remark][29][7]7.29}{[1][53][]54}{}{}{}}
\newlabel{eq:ssgen>0}{{7.16}{54}{}{equation.7.16}{}}
\newlabel{eq:ssgen>0@cref}{{[equation][16][7]7.16}{[1][53][]54}{}{}{}}
\newlabel{eq:BCFW:curve_H1}{{7.17}{54}{\ORATITLE }{equation.7.17}{}}
\newlabel{eq:BCFW:curve_H1@cref}{{[equation][17][7]7.17}{[1][54][]54}{}{}{}}
\newlabel{eq:BCFW:sumbD+sumwD=sumD}{{7.18}{55}{\ORATITLE }{equation.7.18}{}}
\newlabel{eq:BCFW:sumbD+sumwD=sumD@cref}{{[equation][18][7]7.18}{[1][55][]55}{}{}{}}
\newlabel{eq:BCFW:D1_D2_D}{{7.19}{55}{\ORATITLE }{equation.7.19}{}}
\newlabel{eq:BCFW:D1_D2_D@cref}{{[equation][19][7]7.19}{[1][55][]55}{}{}{}}
\newlabel{eq:BCFW:sum_fo_pi}{{7.20}{55}{\ORATITLE }{equation.7.20}{}}
\newlabel{eq:BCFW:sum_fo_pi@cref}{{[equation][20][7]7.20}{[1][55][]55}{}{}{}}
\citation{LPW}
\citation{PSBW}
\citation{LPW}
\citation{origami2}
\citation{AHTT}
\citation{AHT}
\citation{PSBW}
\@writefile{toc}{\contentsline {section}{\tocsection {}{8}{T-duality}}{56}{section.8}\protected@file@percent }
\newlabel{sec:TREE}{{8}{56}{T-duality}{section.8}{}}
\newlabel{sec:TREE@cref}{{[section][8][]8}{[1][56][]56}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\tocsubsection {}{8.1}{T-duality for ambient amplituhedra}}{56}{subsection.8.1}\protected@file@percent }
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~8.1\else \numberline {8.1}Definition\fi }{56}{definition.8.1}\protected@file@percent }
\newlabel{eq:TREE:wind_vs_varx}{{8.1}{56}{T-duality for ambient amplituhedra}{equation.8.1}{}}
\newlabel{eq:TREE:wind_vs_varx@cref}{{[equation][1][8]8.1}{[1][56][]56}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~8.2\else \numberline {8.2}Definition\fi }{56}{definition.8.2}\protected@file@percent }
\newlabel{dfn:TREE:AAkn}{{8.2}{56}{}{definition.8.2}{}}
\newlabel{dfn:TREE:AAkn@cref}{{[definition][2][8]8.2}{[1][56][]56}{}{}{}}
\newlabel{eq:TREE:AAkn_dfn}{{8.2}{56}{}{equation.8.2}{}}
\newlabel{eq:TREE:AAkn_dfn@cref}{{[equation][2][8]8.2}{[1][56][]56}{}{}{}}
\newlabel{eq:TREE:AAddf_dfn}{{8.3}{56}{}{equation.8.3}{}}
\newlabel{eq:TREE:AAddf_dfn@cref}{{[equation][3][8]8.3}{[1][56][]56}{}{}{}}
\newlabel{eq:AAshift_dfn}{{8.4}{56}{T-duality for ambient amplituhedra}{equation.8.4}{}}
\newlabel{eq:AAshift_dfn@cref}{{[equation][4][8]8.4}{[1][56][]56}{}{}{}}
\newlabel{eq:AAiso_dfn}{{8.5}{56}{T-duality for ambient amplituhedra}{equation.8.5}{}}
\newlabel{eq:AAiso_dfn@cref}{{[equation][5][8]8.5}{[1][56][]56}{}{}{}}
\@writefile{loe}{\contentsline {theorem}{\ifthmt@listswap Theorem~8.3\else \numberline {8.3}Theorem\fi \thmtformatoptarg {T-duality for ambient amplituhedra}}{56}{theorem.8.3}\protected@file@percent }
\newlabel{thm:AAshift}{{8.3}{56}{T-duality for ambient amplituhedra}{theorem.8.3}{}}
\newlabel{thm:AAshift@cref}{{[theorem][3][8]8.3}{[1][56][]56}{}{}{}}
\newlabel{AAshift_iso}{{{{(1)}}}{56}{T-duality for ambient amplituhedra}{Item.44}{}}
\newlabel{AAshift_iso@cref}{{[enumi][1][]{{(1)}}}{[1][56][]56}{}{}{}}
\newlabel{AAshift_forg}{{{{(2)}}}{56}{T-duality for ambient amplituhedra}{Item.45}{}}
\newlabel{AAshift_forg@cref}{{[enumi][2][]{{(2)}}}{[1][56][]56}{}{}{}}
\newlabel{ssec:TREE:Mand_vs_Pluck}{{8.2}{57}{\MdashTITLE positivity vs Pl\"ucker-positivity}{subsection.8.2}{}}
\newlabel{ssec:TREE:Mand_vs_Pluck@cref}{{[subsection][2][8]8.2}{[1][56][]57}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\tocsubsection {}{8.2}{Mandelstam-positivity vs Pl\"ucker-positivity}}{57}{subsection.8.2}\protected@file@percent }
\@writefile{loe}{\contentsline {proposition}{\ifthmt@listswap Proposition~8.4\else \numberline {8.4}Proposition\fi }{57}{proposition.8.4}\protected@file@percent }
\newlabel{prop:MPnla_AAnla_homeo}{{8.4}{57}{}{proposition.8.4}{}}
\newlabel{prop:MPnla_AAnla_homeo@cref}{{[proposition][4][8]8.4}{[1][57][]57}{}{}{}}
\newlabel{eq:x_vs_ap_vs_am}{{8.6}{57}{\MdashTITLE positivity vs Pl\"ucker-positivity}{equation.8.6}{}}
\newlabel{eq:x_vs_ap_vs_am@cref}{{[equation][6][8]8.6}{[1][57][]57}{}{}{}}
\newlabel{eq:xM_to_x}{{8.7}{57}{\MdashTITLE positivity vs Pl\"ucker-positivity}{equation.8.7}{}}
\newlabel{eq:xM_to_x@cref}{{[equation][7][8]8.7}{[1][57][]57}{}{}{}}
\newlabel{eq:det_xM_vs_Pmom^2}{{8.8}{57}{\MdashTITLE positivity vs Pl\"ucker-positivity}{equation.8.8}{}}
\newlabel{eq:det_xM_vs_Pmom^2@cref}{{[equation][8][8]8.8}{[1][57][]57}{}{}{}}
\newlabel{eq:TE:decor_dfn}{{8.9}{57}{\MdashTITLE positivity vs Pl\"ucker-positivity}{equation.8.9}{}}
\newlabel{eq:TE:decor_dfn@cref}{{[equation][9][8]8.9}{[1][57][]57}{}{}{}}
\newlabel{eq:brV_vs_Mand}{{8.10}{58}{\MdashTITLE positivity vs Pl\"ucker-positivity}{equation.8.10}{}}
\newlabel{eq:brV_vs_Mand@cref}{{[equation][10][8]8.10}{[1][57][]58}{}{}{}}
\newlabel{eq:TREE:brV_calc_brla}{{8.11}{58}{\MdashTITLE positivity vs Pl\"ucker-positivity}{equation.8.11}{}}
\newlabel{eq:TREE:brV_calc_brla@cref}{{[equation][11][8]8.11}{[1][58][]58}{}{}{}}
\@writefile{loe}{\contentsline {remark}{\ifthmt@listswap Remark~8.5\else \numberline {8.5}Remark\fi }{58}{remark.8.5}\protected@file@percent }
\newlabel{rmk:Mand=>brlat>0}{{8.5}{58}{}{remark.8.5}{}}
\newlabel{rmk:Mand=>brlat>0@cref}{{[remark][5][8]8.5}{[1][58][]58}{}{}{}}
\@writefile{loe}{\contentsline {notation}{\ifthmt@listswap Notation~8.6\else \numberline {8.6}Notation\fi }{58}{notation.8.6}\protected@file@percent }
\newlabel{eq:V_la_mu_lat}{{8.12}{58}{}{equation.8.12}{}}
\newlabel{eq:V_la_mu_lat@cref}{{[equation][12][8]8.12}{[1][58][]58}{}{}{}}
\newlabel{eq:bdxM_CMI_laii=muii}{{8.13}{58}{\MdashTITLE positivity vs Pl\"ucker-positivity}{equation.8.13}{}}
\newlabel{eq:bdxM_CMI_laii=muii@cref}{{[equation][13][8]8.13}{[1][58][]58}{}{}{}}
\newlabel{eq:Schur_comp}{{8.14}{58}{\MdashTITLE positivity vs Pl\"ucker-positivity}{equation.8.14}{}}
\newlabel{eq:Schur_comp@cref}{{[equation][14][8]8.14}{[1][58][]58}{}{}{}}
\newlabel{eq:windskip_dfn}{{8.15}{58}{\MdashTITLE positivity vs Pl\"ucker-positivity}{equation.8.15}{}}
\newlabel{eq:windskip_dfn@cref}{{[equation][15][8]8.15}{[1][58][]58}{}{}{}}
\newlabel{eq:windskip_vs_varxxx}{{8.16}{58}{\MdashTITLE positivity vs Pl\"ucker-positivity}{equation.8.16}{}}
\newlabel{eq:windskip_vs_varxxx@cref}{{[equation][16][8]8.16}{[1][58][]58}{}{}{}}
\newlabel{eq:wind_la_lat_vs_TURN}{{8.17}{58}{\MdashTITLE positivity vs Pl\"ucker-positivity}{equation.8.17}{}}
\newlabel{eq:wind_la_lat_vs_TURN@cref}{{[equation][17][8]8.17}{[1][58][]58}{}{}{}}
\newlabel{ssec:GLp_winding}{{8.3}{58}{$\GLp $-\winding numbers}{subsection.8.3}{}}
\newlabel{ssec:GLp_winding@cref}{{[subsection][3][8]8.3}{[1][58][]58}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\tocsubsection {}{8.3}{$\operatorname  {GL}_2^+({\mathbb  {R}})$-winding\xspace  numbers}}{58}{subsection.8.3}\protected@file@percent }
\@writefile{loe}{\contentsline {remark}{\ifthmt@listswap Remark~8.7\else \numberline {8.7}Remark\fi }{58}{remark.8.7}\protected@file@percent }
\newlabel{rmk:turnGL_act}{{8.7}{58}{}{remark.8.7}{}}
\newlabel{rmk:turnGL_act@cref}{{[remark][7][8]8.7}{[1][58][]58}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~8.8\else \numberline {8.8}Definition\fi }{58}{definition.8.8}\protected@file@percent }
\newlabel{dfn:GLPath}{{8.8}{58}{}{definition.8.8}{}}
\newlabel{dfn:GLPath@cref}{{[definition][8][8]8.8}{[1][58][]58}{}{}{}}
\citation{Eckmann_Hilton}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~8.9\else \numberline {8.9}Definition\fi }{59}{definition.8.9}\protected@file@percent }
\newlabel{dfn:matrix_null_poly}{{8.9}{59}{}{definition.8.9}{}}
\newlabel{dfn:matrix_null_poly@cref}{{[definition][9][8]8.9}{[1][58][]59}{}{}{}}
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~8.10\else \numberline {8.10}Lemma\fi }{59}{lemma.8.10}\protected@file@percent }
\newlabel{lemma:turnGL_trT}{{8.10}{59}{}{lemma.8.10}{}}
\newlabel{lemma:turnGL_trT@cref}{{[lemma][10][8]8.10}{[1][59][]59}{}{}{}}
\newlabel{eq:muof(ys)_dfn}{{8.18}{59}{$\GLp $-\winding numbers}{equation.8.18}{}}
\newlabel{eq:muof(ys)_dfn@cref}{{[equation][18][8]8.18}{[1][59][]59}{}{}{}}
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~8.11\else \numberline {8.11}Lemma\fi }{59}{lemma.8.11}\protected@file@percent }
\newlabel{eq:windaround_muof}{{8.19}{59}{}{equation.8.19}{}}
\newlabel{eq:windaround_muof@cref}{{[equation][19][8]8.19}{[1][59][]59}{}{}{}}
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~8.12\else \numberline {8.12}Lemma\fi }{59}{lemma.8.12}\protected@file@percent }
\newlabel{eq:varx_muof=varx_brVLy}{{8.20}{59}{}{equation.8.20}{}}
\newlabel{eq:varx_muof=varx_brVLy@cref}{{[equation][20][8]8.20}{[1][59][]59}{}{}{}}
\@writefile{loe}{\contentsline {corollary}{\ifthmt@listswap Corollary~8.13\else \numberline {8.13}Corollary\fi }{59}{corollary.8.13}\protected@file@percent }
\newlabel{cor:var_vs_inside}{{8.13}{59}{}{corollary.8.13}{}}
\newlabel{cor:var_vs_inside@cref}{{[corollary][13][8]8.13}{[1][59][]59}{}{}{}}
\newlabel{eq:var_vs_inside}{{8.21}{59}{}{equation.8.21}{}}
\newlabel{eq:var_vs_inside@cref}{{[equation][21][8]8.21}{[1][59][]59}{}{}{}}
\newlabel{ssec:TREE:proof_thm_AAshift}{{8.4}{60}{Proof of Theorem~\ref {thm:AAshift}}{subsection.8.4}{}}
\newlabel{ssec:TREE:proof_thm_AAshift@cref}{{[subsection][4][8]8.4}{[1][59][]60}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\tocsubsection {}{8.4}{Proof of Theorem~\ref {thm:AAshift}}}{60}{subsection.8.4}\protected@file@percent }
\newlabel{eq:brlae_Arg_lae}{{8.22}{61}{Proof of Theorem~\ref {thm:AAshift}}{equation.8.22}{}}
\newlabel{eq:brlae_Arg_lae@cref}{{[equation][22][8]8.22}{[1][61][]61}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\tocsubsection {}{8.5}{Properties of $\mathcal  {R}$-tilings\xspace  }}{61}{subsection.8.5}\protected@file@percent }
\@writefile{loe}{\contentsline {proposition}{\ifthmt@listswap Proposition~8.14\else \numberline {8.14}Proposition\fi }{61}{proposition.8.14}\protected@file@percent }
\newlabel{lemma:RX_triple}{{8.14}{61}{}{proposition.8.14}{}}
\newlabel{lemma:RX_triple@cref}{{[proposition][14][8]8.14}{[1][61][]61}{}{}{}}
\newlabel{eq:TREE:comm_diag}{{8.23}{61}{}{equation.8.23}{}}
\newlabel{eq:TREE:comm_diag@cref}{{[equation][23][8]8.23}{[1][61][]61}{}{}{}}
\newlabel{eq:RtilingS}{{8.24}{61}{}{equation.8.24}{}}
\newlabel{eq:RtilingS@cref}{{[equation][24][8]8.24}{[1][61][]61}{}{}{}}
\newlabel{eq:ReloB_vs_ReloC_Cartesian}{{8.25}{61}{Properties of \mtilings }{equation.8.25}{}}
\newlabel{eq:ReloB_vs_ReloC_Cartesian@cref}{{[equation][25][8]8.25}{[1][61][]61}{}{}{}}
\newlabel{eq:TREE:comm_diag_res}{{8.26}{62}{Properties of \mtilings }{equation.8.26}{}}
\newlabel{eq:TREE:comm_diag_res@cref}{{[equation][26][8]8.26}{[1][61][]62}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~8.15\else \numberline {8.15}Definition\fi \thmtformatoptarg {Tiling}}{62}{definition.8.15}\protected@file@percent }
\newlabel{dfn:BCFW:tiling}{{8.15}{62}{Tiling}{definition.8.15}{}}
\newlabel{dfn:BCFW:tiling@cref}{{[definition][15][8]8.15}{[1][62][]62}{}{}{}}
\newlabel{tiling1}{{{{(a)}}}{62}{Tiling}{Item.46}{}}
\newlabel{tiling1@cref}{{[enumi][1][]{{(a)}}}{[1][62][]62}{}{}{}}
\newlabel{tiling2}{{{{(b)}}}{62}{Tiling}{Item.47}{}}
\newlabel{tiling2@cref}{{[enumi][2][]{{(b)}}}{[1][62][]62}{}{}{}}
\newlabel{tiling3}{{{{(c)}}}{62}{Tiling}{Item.48}{}}
\newlabel{tiling3@cref}{{[enumi][3][]{{(c)}}}{[1][62][]62}{}{}{}}
\@writefile{loe}{\contentsline {proposition}{\ifthmt@listswap Proposition~8.16\else \numberline {8.16}Proposition\fi }{62}{proposition.8.16}\protected@file@percent }
\newlabel{lemma:Rtiling_to_tiling}{{8.16}{62}{}{proposition.8.16}{}}
\newlabel{lemma:Rtiling_to_tiling@cref}{{[proposition][16][8]8.16}{[1][62][]62}{}{}{}}
\newlabel{eq:RGraph}{{8.27}{62}{}{equation.8.27}{}}
\newlabel{eq:RGraph@cref}{{[equation][27][8]8.27}{[1][62][]62}{}{}{}}
\citation{AHTT}
\citation{HZ_notes}
\citation{DFLP}
\citation{AHT}
\citation{DFLP}
\newlabel{eq:RWo=RYo_cap_RW}{{8.28}{63}{Properties of \mtilings }{equation.8.28}{}}
\newlabel{eq:RWo=RYo_cap_RW@cref}{{[equation][28][8]8.28}{[1][62][]63}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\tocsubsection {}{8.6}{T-duality for ambient amplituhedron tilings}}{63}{subsection.8.6}\protected@file@percent }
\newlabel{eq:RXA_dfn}{{8.29}{63}{T-duality for ambient amplituhedron tilings}{equation.8.29}{}}
\newlabel{eq:RXA_dfn@cref}{{[equation][29][8]8.29}{[1][63][]63}{}{}{}}
\newlabel{eq:RXB_dfn}{{8.30}{63}{T-duality for ambient amplituhedron tilings}{equation.8.30}{}}
\newlabel{eq:RXB_dfn@cref}{{[equation][30][8]8.30}{[1][63][]63}{}{}{}}
\newlabel{eq:RXC_dfn}{{8.31}{63}{T-duality for ambient amplituhedron tilings}{equation.8.31}{}}
\newlabel{eq:RXC_dfn@cref}{{[equation][31][8]8.31}{[1][63][]63}{}{}{}}
\@writefile{loe}{\contentsline {remark}{\ifthmt@listswap Remark~8.17\else \numberline {8.17}Remark\fi }{63}{remark.8.17}\protected@file@percent }
\@writefile{loe}{\contentsline {corollary}{\ifthmt@listswap Corollary~8.18\else \numberline {8.18}Corollary\fi \thmtformatoptarg {T-duality for $\mathcal  {R}$-tilings\xspace  of ambient amplituhedra}}{63}{corollary.8.18}\protected@file@percent }
\newlabel{lemma:TREE:amb_tiling_equivalence}{{8.18}{63}{T-duality for \mtilings of ambient amplituhedra}{corollary.8.18}{}}
\newlabel{lemma:TREE:amb_tiling_equivalence@cref}{{[corollary][18][8]8.18}{[1][63][]63}{}{}{}}
\@writefile{loe}{\contentsline {corollary}{\ifthmt@listswap Corollary~8.19\else \numberline {8.19}Corollary\fi }{63}{corollary.8.19}\protected@file@percent }
\newlabel{lemma:ddf_triang}{{8.19}{63}{}{corollary.8.19}{}}
\newlabel{lemma:ddf_triang@cref}{{[corollary][19][8]8.19}{[1][63][]63}{}{}{}}
\citation{HZ_notes}
\citation{DFLP}
\citation{KW}
\citation{AHTT}
\citation{AHTT}
\citation{DFLP}
\@writefile{toc}{\contentsline {subsection}{\tocsubsection {}{8.7}{Sign flip and linear projection amplituhedra}}{64}{subsection.8.7}\protected@file@percent }
\newlabel{eq:PsiZ_dfn}{{8.32}{64}{Sign flip and linear projection amplituhedra}{equation.8.32}{}}
\newlabel{eq:PsiZ_dfn@cref}{{[equation][32][8]8.32}{[1][64][]64}{}{}{}}
\@writefile{loe}{\contentsline {remark}{\ifthmt@listswap Remark~8.20\else \numberline {8.20}Remark\fi }{64}{remark.8.20}\protected@file@percent }
\newlabel{rmk:dim_ddC_cap_Z=4}{{8.20}{64}{}{remark.8.20}{}}
\newlabel{rmk:dim_ddC_cap_Z=4@cref}{{[remark][20][8]8.20}{[1][64][]64}{}{}{}}
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~8.21\else \numberline {8.21}Lemma\fi }{64}{lemma.8.21}\protected@file@percent }
\newlabel{lemma:TREE:proj_subset_amb}{{8.21}{64}{}{lemma.8.21}{}}
\newlabel{lemma:TREE:proj_subset_amb@cref}{{[lemma][21][8]8.21}{[1][64][]64}{}{}{}}
\newlabel{eq:TREE:proj_subset_cl_amb}{{8.33}{64}{}{equation.8.33}{}}
\newlabel{eq:TREE:proj_subset_cl_amb@cref}{{[equation][33][8]8.33}{[1][64][]64}{}{}{}}
\@writefile{loe}{\contentsline {theorem}{\ifthmt@listswap Theorem~8.22\else \numberline {8.22}Theorem\fi \thmtformatoptarg {BCFW tilings of amplituhedra}}{64}{theorem.8.22}\protected@file@percent }
\newlabel{lemma:proj_tiling}{{8.22}{64}{BCFW tilings of amplituhedra}{theorem.8.22}{}}
\newlabel{lemma:proj_tiling@cref}{{[theorem][22][8]8.22}{[1][64][]64}{}{}{}}
\newlabel{proj_tiling1}{{{{(1)}}}{64}{BCFW tilings of amplituhedra}{Item.49}{}}
\newlabel{proj_tiling1@cref}{{[enumi][1][]{{(1)}}}{[1][64][]64}{}{}{}}
\newlabel{proj_tiling2}{{{{(2)}}}{64}{BCFW tilings of amplituhedra}{Item.50}{}}
\newlabel{proj_tiling2@cref}{{[enumi][2][]{{(2)}}}{[1][64][]64}{}{}{}}
\newlabel{proj_tiling3}{{{{(3)}}}{64}{BCFW tilings of amplituhedra}{Item.51}{}}
\newlabel{proj_tiling3@cref}{{[enumi][3][]{{(3)}}}{[1][64][]64}{}{}{}}
\newlabel{eq:TREE:proj=cl_amb}{{8.34}{64}{BCFW tilings of amplituhedra}{equation.8.34}{}}
\newlabel{eq:TREE:proj=cl_amb@cref}{{[equation][34][8]8.34}{[1][64][]64}{}{}{}}
\citation{KW}
\citation{ELT}
\citation{ELPTSBW}
\citation{ELT}
\citation{ELPTSBW}
\citation{ELT}
\citation{ELPTSBW}
\citation{origami2}
\newlabel{eq:KW_eq}{{8.35}{65}{Sign flip and linear projection amplituhedra}{equation.8.35}{}}
\newlabel{eq:KW_eq@cref}{{[equation][35][8]8.35}{[1][65][]65}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\tocsubsection {}{8.8}{Discussion}}{65}{subsection.8.8}\protected@file@percent }
\@writefile{loe}{\contentsline {remark}{\ifthmt@listswap Remark~8.23\else \numberline {8.23}Remark\fi }{65}{remark.8.23}\protected@file@percent }
\newlabel{rmk:msgen_exist}{{8.23}{65}{}{remark.8.23}{}}
\newlabel{rmk:msgen_exist@cref}{{[remark][23][8]8.23}{[1][65][]65}{}{}{}}
\@writefile{loe}{\contentsline {remark}{\ifthmt@listswap Remark~8.24\else \numberline {8.24}Remark\fi }{65}{remark.8.24}\protected@file@percent }
\newlabel{rmk:converse_main_diff}{{8.24}{65}{}{remark.8.24}{}}
\newlabel{rmk:converse_main_diff@cref}{{[remark][24][8]8.24}{[1][65][]65}{}{}{}}
\@writefile{loe}{\contentsline {question}{\ifthmt@listswap Question~8.25\else \numberline {8.25}Question\fi }{65}{question.8.25}\protected@file@percent }
\newlabel{que:TREE:extend}{{8.25}{65}{}{question.8.25}{}}
\newlabel{que:TREE:extend@cref}{{[question][25][8]8.25}{[1][65][]65}{}{}{}}
\@writefile{loe}{\contentsline {remark}{\ifthmt@listswap Remark~8.26\else \numberline {8.26}Remark\fi }{65}{remark.8.26}\protected@file@percent }
\newlabel{rmk:ELT_ELPTSBW}{{8.26}{65}{}{remark.8.26}{}}
\newlabel{rmk:ELT_ELPTSBW@cref}{{[remark][26][8]8.26}{[1][65][]65}{}{}{}}
\citation{origami2}
\citation{GL_parity}
\citation{GL_parity}
\citation{MuSp}
\citation{MuSp}
\citation{GL_parity}
\citation{CLR2}
\citation{CLR2}
\@writefile{loe}{\contentsline {remark}{\ifthmt@listswap Remark~8.27\else \numberline {8.27}Remark\fi }{66}{remark.8.27}\protected@file@percent }
\newlabel{eq:SHIFT:Muni-Auni}{{8.36}{66}{}{equation.8.36}{}}
\newlabel{eq:SHIFT:Muni-Auni@cref}{{[equation][36][8]8.36}{[1][66][]66}{}{}{}}
\@writefile{loe}{\contentsline {remark}{\ifthmt@listswap Remark~8.28\else \numberline {8.28}Remark\fi \thmtformatoptarg {Parity duality}}{66}{remark.8.28}\protected@file@percent }
\@writefile{toc}{\contentsline {section}{\tocsection {}{9}{Perfect t-embeddings}}{66}{section.9}\protected@file@percent }
\newlabel{sec:perf}{{9}{66}{Perfect t-embeddings}{section.9}{}}
\newlabel{sec:perf@cref}{{[section][9][]9}{[1][66][]66}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~9.1\else \numberline {9.1}Definition\fi }{66}{definition.9.1}\protected@file@percent }
\newlabel{dfn:perf}{{9.1}{66}{}{definition.9.1}{}}
\newlabel{dfn:perf@cref}{{[definition][1][9]9.1}{[1][66][]66}{}{}{}}
\newlabel{perf1}{{{{(i)}}}{66}{}{Item.54}{}}
\newlabel{perf1@cref}{{[enumi][1][]{{(i)}}}{[1][66][]66}{}{}{}}
\newlabel{perf2}{{{{(ii)}}}{66}{}{Item.55}{}}
\newlabel{perf2@cref}{{[enumi][2][]{{(ii)}}}{[1][66][]66}{}{}{}}
\@writefile{loe}{\contentsline {remark}{\ifthmt@listswap Remark~9.2\else \numberline {9.2}Remark\fi }{66}{remark.9.2}\protected@file@percent }
\newlabel{rmk:n_even}{{9.2}{66}{}{remark.9.2}{}}
\newlabel{rmk:n_even@cref}{{[remark][2][9]9.2}{[1][66][]66}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\tocsubsection {}{9.1}{An involution}}{67}{subsection.9.1}\protected@file@percent }
\newlabel{eq:pinv(la)_dfn}{{9.1}{67}{An involution}{equation.9.1}{}}
\newlabel{eq:pinv(la)_dfn@cref}{{[equation][1][9]9.1}{[1][66][]67}{}{}{}}
\newlabel{eq:perf:tlai_dfn}{{9.2}{67}{An involution}{equation.9.2}{}}
\newlabel{eq:perf:tlai_dfn@cref}{{[equation][2][9]9.2}{[1][66][]67}{}{}{}}
\newlabel{eq:perf:pinv_dfn_mat}{{9.3}{67}{An involution}{equation.9.3}{}}
\newlabel{eq:perf:pinv_dfn_mat@cref}{{[equation][3][9]9.3}{[1][67][]67}{}{}{}}
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~9.3\else \numberline {9.3}Lemma\fi }{67}{lemma.9.3}\protected@file@percent }
\newlabel{lemma:perf:pinv}{{9.3}{67}{}{lemma.9.3}{}}
\newlabel{lemma:perf:pinv@cref}{{[lemma][3][9]9.3}{[1][67][]67}{}{}{}}
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~9.4\else \numberline {9.4}Lemma\fi }{67}{lemma.9.4}\protected@file@percent }
\newlabel{lemma:perfect=>MP_and_n=2k}{{9.4}{67}{}{lemma.9.4}{}}
\newlabel{lemma:perfect=>MP_and_n=2k@cref}{{[lemma][4][9]9.4}{[1][67][]67}{}{}{}}
\newlabel{eq:Mand_perfect_formula}{{9.4}{67}{An involution}{equation.9.4}{}}
\newlabel{eq:Mand_perfect_formula@cref}{{[equation][4][9]9.4}{[1][67][]67}{}{}{}}
\@writefile{loe}{\contentsline {proposition}{\ifthmt@listswap Proposition~9.5\else \numberline {9.5}Proposition\fi }{67}{proposition.9.5}\protected@file@percent }
\newlabel{prop:perfect}{{9.5}{67}{}{proposition.9.5}{}}
\newlabel{prop:perfect@cref}{{[proposition][5][9]9.5}{[1][67][]67}{}{}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {14}{\ignorespaces  A weighted hexagonal prism $(\Gamma ,\operatorname  {wt})$ with unmarked edges having weight $1$ and two perfect t-embeddings of $(\Gamma ,\operatorname  {wt})$; see \cref  {rmk:CLR_outer_face}.}}{68}{figure.caption.18}\protected@file@percent }
\newlabel{fig:hex}{{14}{68}{A weighted hexagonal prism $(\G ,\wt )$ with unmarked edges having weight $1$ and two perfect t-embeddings of $(\G ,\wt )$; see \cref {rmk:CLR_outer_face}}{figure.caption.18}{}}
\newlabel{fig:hex@cref}{{[figure][14][]14}{[1][68][]68}{}{}{}}
\@writefile{loe}{\contentsline {remark}{\ifthmt@listswap Remark~9.6\else \numberline {9.6}Remark\fi }{68}{remark.9.6}\protected@file@percent }
\newlabel{rmk:perf_Lorentz}{{9.6}{68}{}{remark.9.6}{}}
\newlabel{rmk:perf_Lorentz@cref}{{[remark][6][9]9.6}{[1][68][]68}{}{}{}}
\@writefile{loe}{\contentsline {corollary}{\ifthmt@listswap Corollary~9.7\else \numberline {9.7}Corollary\fi }{68}{corollary.9.7}\protected@file@percent }
\newlabel{cor:perf:n=2k}{{9.7}{68}{}{corollary.9.7}{}}
\newlabel{cor:perf:n=2k@cref}{{[corollary][7][9]9.7}{[1][68][]68}{}{}{}}
\newlabel{ssec:T_dual_perfect}{{9.2}{68}{T-dual perfect t-embeddings}{subsection.9.2}{}}
\newlabel{ssec:T_dual_perfect@cref}{{[subsection][2][9]9.2}{[1][68][]68}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\tocsubsection {}{9.2}{T-dual perfect t-embeddings}}{68}{subsection.9.2}\protected@file@percent }
\@writefile{loe}{\contentsline {proposition}{\ifthmt@listswap Proposition~9.8\else \numberline {9.8}Proposition\fi }{68}{proposition.9.8}\protected@file@percent }
\newlabel{prop:T_dual_perfect_vs_perfect}{{9.8}{68}{}{proposition.9.8}{}}
\newlabel{prop:T_dual_perfect_vs_perfect@cref}{{[proposition][8][9]9.8}{[1][68][]68}{}{}{}}
\newlabel{eq:perfect_V}{{9.5}{68}{}{equation.9.5}{}}
\newlabel{eq:perfect_V@cref}{{[equation][5][9]9.5}{[1][68][]68}{}{}{}}
\citation{origami2}
\newlabel{eq:perfect_alt_oplus_dim4}{{9.6}{69}{T-dual perfect t-embeddings}{equation.9.6}{}}
\newlabel{eq:perfect_alt_oplus_dim4@cref}{{[equation][6][9]9.6}{[1][68][]69}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~9.9\else \numberline {9.9}Definition\fi }{69}{definition.9.9}\protected@file@percent }
\@writefile{loe}{\contentsline {corollary}{\ifthmt@listswap Corollary~9.10\else \numberline {9.10}Corollary\fi }{69}{corollary.9.10}\protected@file@percent }
\newlabel{rmk:from_T_dual_perfect_to_perfect}{{9.10}{69}{}{corollary.9.10}{}}
\newlabel{rmk:from_T_dual_perfect_to_perfect@cref}{{[corollary][10][9]9.10}{[1][69][]69}{}{}{}}
\@writefile{loe}{\contentsline {remark}{\ifthmt@listswap Remark~9.11\else \numberline {9.11}Remark\fi }{69}{remark.9.11}\protected@file@percent }
\@writefile{loe}{\contentsline {remark}{\ifthmt@listswap Remark~9.12\else \numberline {9.12}Remark\fi }{69}{remark.9.12}\protected@file@percent }
\citation{Skandera}
\citation{Farber_Postnikov}
\citation{GL_parity}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~9.13\else \numberline {9.13}Definition\fi }{70}{definition.9.13}\protected@file@percent }
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~9.14\else \numberline {9.14}Lemma\fi \thmtformatoptarg {\cite  [Theorem~6.3]{Farber_Postnikov}}}{70}{lemma.9.14}\protected@file@percent }
\newlabel{lemma:oend_Skandera}{{9.14}{70}{\cite [Theorem~6.3]{Farber_Postnikov}}{lemma.9.14}{}}
\newlabel{lemma:oend_Skandera@cref}{{[lemma][14][9]9.14}{[1][70][]70}{}{}{}}
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~9.15\else \numberline {9.15}Definition\fi }{70}{definition.9.15}\protected@file@percent }
\newlabel{dfn:Catalan}{{9.15}{70}{}{definition.9.15}{}}
\newlabel{dfn:Catalan@cref}{{[definition][15][9]9.15}{[1][70][]70}{}{}{}}
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~9.16\else \numberline {9.16}Lemma\fi }{70}{lemma.9.16}\protected@file@percent }
\newlabel{lemma:oend_Catalan}{{9.16}{70}{}{lemma.9.16}{}}
\newlabel{lemma:oend_Catalan@cref}{{[lemma][16][9]9.16}{[1][70][]70}{}{}{}}
\@writefile{loe}{\contentsline {theorem}{\ifthmt@listswap Theorem~9.17\else \numberline {9.17}Theorem\fi \thmtformatoptarg {Existence and uniqueness of T-dual perfect t-embeddings}}{70}{theorem.9.17}\protected@file@percent }
\newlabel{thm:T_dual_perfect}{{9.17}{70}{Existence and uniqueness of T-dual perfect t-embeddings}{theorem.9.17}{}}
\newlabel{thm:T_dual_perfect@cref}{{[theorem][17][9]9.17}{[1][70][]70}{}{}{}}
\newlabel{eq:V_vs_ddC_cap}{{9.7}{70}{Existence and uniqueness of T-dual perfect t-embeddings}{equation.9.7}{}}
\newlabel{eq:V_vs_ddC_cap@cref}{{[equation][7][9]9.7}{[1][70][]70}{}{}{}}
\citation{CLR2}
\citation{CLR2}
\@writefile{loe}{\contentsline {corollary}{\ifthmt@listswap Corollary~9.18\else \numberline {9.18}Corollary\fi \thmtformatoptarg {Existence of perfect t-embeddings}}{71}{corollary.9.18}\protected@file@percent }
\newlabel{lemma:perfect_exist_G}{{9.18}{71}{Existence of perfect t-embeddings}{corollary.9.18}{}}
\newlabel{lemma:perfect_exist_G@cref}{{[corollary][18][9]9.18}{[1][71][]71}{}{}{}}
\@writefile{loe}{\contentsline {remark}{\ifthmt@listswap Remark~9.19\else \numberline {9.19}Remark\fi }{71}{remark.9.19}\protected@file@percent }
\newlabel{rmk:perfect_diagram}{{9.19}{71}{}{remark.9.19}{}}
\newlabel{rmk:perfect_diagram@cref}{{[remark][19][9]9.19}{[1][71][]71}{}{}{}}
\newlabel{eq:MPerf_dfn}{{9.8}{71}{}{equation.9.8}{}}
\newlabel{eq:MPerf_dfn@cref}{{[equation][8][9]9.8}{[1][71][]71}{}{}{}}
\newlabel{eq:Aperf_dfn}{{9.9}{71}{}{equation.9.9}{}}
\newlabel{eq:Aperf_dfn@cref}{{[equation][9][9]9.9}{[1][71][]71}{}{}{}}
\newlabel{eq:perf_proj}{{9.10}{71}{}{equation.9.10}{}}
\newlabel{eq:perf_proj@cref}{{[equation][10][9]9.10}{[1][71][]71}{}{}{}}
\@writefile{loe}{\contentsline {question}{\ifthmt@listswap Question~9.20\else \numberline {9.20}Question\fi }{71}{question.9.20}\protected@file@percent }
\@writefile{loe}{\contentsline {question}{\ifthmt@listswap Question~9.21\else \numberline {9.21}Question\fi }{71}{question.9.21}\protected@file@percent }
\newlabel{ssec:perfect_neg}{{9.3}{71}{Negative results on existence and uniqueness of perfect t-embeddings}{subsection.9.3}{}}
\newlabel{ssec:perfect_neg@cref}{{[subsection][3][9]9.3}{[1][71][]71}{}{}{}}
\@writefile{toc}{\contentsline {subsection}{\tocsubsection {}{9.3}{Negative results on existence and uniqueness of perfect t-embeddings}}{71}{subsection.9.3}\protected@file@percent }
\newlabel{eq:perf:perp}{{9.11}{71}{Negative results on existence and uniqueness of perfect t-embeddings}{equation.9.11}{}}
\newlabel{eq:perf:perp@cref}{{[equation][11][9]9.11}{[1][71][]71}{}{}{}}
\citation{CLR2}
\citation{CLR2}
\citation{Chelkak_s_emb}
\citation{OPT}
\citation{Huang_Wen}
\citation{Huang_Wen_Xie}
\citation{GP_Ising}
\@writefile{loe}{\contentsline {example}{\ifthmt@listswap Example~9.22\else \numberline {9.22}Example\fi }{72}{example.9.22}\protected@file@percent }
\newlabel{ex:perf:two_solutions}{{9.22}{72}{}{example.9.22}{}}
\newlabel{ex:perf:two_solutions@cref}{{[example][22][9]9.22}{[1][71][]72}{}{}{}}
\@writefile{loe}{\contentsline {remark}{\ifthmt@listswap Remark~9.23\else \numberline {9.23}Remark\fi }{72}{remark.9.23}\protected@file@percent }
\newlabel{rmk:CLR_outer_face}{{9.23}{72}{}{remark.9.23}{}}
\newlabel{rmk:CLR_outer_face@cref}{{[remark][23][9]9.23}{[1][72][]72}{}{}{}}
\@writefile{loe}{\contentsline {lemma}{\ifthmt@listswap Lemma~9.24\else \numberline {9.24}Lemma\fi }{72}{lemma.9.24}\protected@file@percent }
\newlabel{lemma:perf:no_solutions}{{9.24}{72}{}{lemma.9.24}{}}
\newlabel{lemma:perf:no_solutions@cref}{{[lemma][24][9]9.24}{[1][72][]72}{}{}{}}
\@writefile{loe}{\contentsline {remark}{\ifthmt@listswap Remark~9.25\else \numberline {9.25}Remark\fi }{72}{remark.9.25}\protected@file@percent }
\@writefile{toc}{\contentsline {section}{\tocsection {Appendix}{A}{ABJM amplituhedra, s-embeddings, and the problem of Apollonius}}{72}{appendix.A}\protected@file@percent }
\newlabel{sec:ABJM}{{A}{72}{ABJM amplituhedra, s-embeddings, and the problem of Apollonius}{appendix.A}{}}
\newlabel{sec:ABJM@cref}{{[section][1][]A}{[1][72][]72}{}{}{}}
\@writefile{loe}{\contentsline {remark}{\ifthmt@listswap Remark~A.1\else \numberline {A.1}Remark\fi }{72}{remark.A.1}\protected@file@percent }
\@writefile{toc}{\contentsline {subsection}{\tocsubsection {}{A.1}{ABJM momentum amplituhedron and Ising model}}{72}{subsection.A.1}\protected@file@percent }
\@writefile{loe}{\contentsline {definition}{\ifthmt@listswap Definition~A.2\else \numberline {A.2}Definition\fi }{72}{definition.A.2}\protected@file@percent }
\newlabel{eq:MBJk_dfn}{{A.1}{72}{}{equation.A.1}{}}
\newlabel{eq:MBJk_dfn@cref}{{[equation][1][1]A.1}{[1][72][]72}{}{}{}}
\citation{Dubedat}
\citation{Huang_Wen}
\citation{GP_Ising}
\citation{Chelkak_s_emb}
\citation{CLR1}
\citation{OPT}
\citation{Huang_Wen}
\citation{GP_Ising}
\@writefile{loe}{\contentsline {remark}{\ifthmt@listswap Remark~A.3\else \numberline {A.3}Remark\fi }{73}{remark.A.3}\protected@file@percent }
\newlabel{rmk:ABJM_vs_perf}{{A.3}{73}{}{remark.A.3}{}}
\newlabel{rmk:ABJM_vs_perf@cref}{{[remark][3][1]A.3}{[1][73][]73}{}{}{}}
\@writefile{loe}{\contentsline {remark}{\ifthmt@listswap Remark~A.4\else \numberline {A.4}Remark\fi \thmtformatoptarg {Existence of s-embeddings}}{73}{remark.A.4}\protected@file@percent }
\@writefile{toc}{\contentsline {subsection}{\tocsubsection {}{A.2}{BCFW recursion and problem of Apollonius}}{73}{subsection.A.2}\protected@file@percent }
\newlabel{eq:C_JIS}{{A.2}{73}{BCFW recursion and problem of Apollonius}{equation.A.2}{}}
\newlabel{eq:C_JIS@cref}{{[equation][2][1]A.2}{[1][73][]73}{}{}{}}
\@writefile{lof}{\contentsline {figure}{\numberline {15}{\ignorespaces  An ABJM origami reconstruction step\xspace  . Compare with \cref  {fig:BCFW}.}}{74}{figure.caption.19}\protected@file@percent }
\newlabel{fig:ABJM}{{15}{74}{An ABJM \ORst . Compare with \cref {fig:BCFW}}{figure.caption.19}{}}
\newlabel{fig:ABJM@cref}{{[figure][15][]15}{[1][73][]74}{}{}{}}
\newlabel{ABJM_summ1}{{{{(1)}}}{74}{BCFW recursion and problem of Apollonius}{Item.60}{}}
\newlabel{ABJM_summ1@cref}{{[enumi][1][]{{(1)}}}{[1][74][]74}{}{}{}}
\newlabel{ABJM_summ2}{{{{(2)}}}{74}{BCFW recursion and problem of Apollonius}{Item.61}{}}
\newlabel{ABJM_summ2@cref}{{[enumi][2][]{{(2)}}}{[1][74][]74}{}{}{}}
\newlabel{ABJM_summ3}{{{{(3)}}}{74}{BCFW recursion and problem of Apollonius}{Item.62}{}}
\newlabel{ABJM_summ3@cref}{{[enumi][3][]{{(3)}}}{[1][74][]74}{}{}{}}
\citation{KLRR}
\citation{Varchenko}
\citation{OrTe}
\citation{CHY1}
\citation{Lam_moduli}
\citation{Stanley_hyp}
\@writefile{lof}{\contentsline {figure}{\numberline {16}{\ignorespaces  The hyperplane arrangement $\overline  {\mathcal  {A}}_C$ for $C$ as in \cref  {ex:Varc1} (left). The $\beta (C)=5$ t-embeddings with prescribed boundary (right).}}{76}{figure.caption.20}\protected@file@percent }
\newlabel{fig:Varc}{{16}{76}{The hyperplane arrangement $\bHArrC $ for $C$ as in \cref {ex:Varc1} (left). The $\bbar (C)=5$ t-embeddings with prescribed boundary (right)}{figure.caption.20}{}}
\newlabel{fig:Varc@cref}{{[figure][16][]16}{[1][76][]76}{}{}{}}
\@writefile{toc}{\contentsline {section}{\tocsection {Appendix}{B}{T-embeddings~with~prescribed~boundary and positroid hyperplane arrangements}}{76}{appendix.B}\protected@file@percent }
\newlabel{sec:Varc}{{B}{76}{T-embeddings~with~prescribed~boundary and positroid hyperplane arrangements}{appendix.B}{}}
\newlabel{sec:Varc@cref}{{[section][2][]B}{[1][76][]76}{}{}{}}
\@writefile{loe}{\contentsline {example}{\ifthmt@listswap Example~B.1\else \numberline {B.1}Example\fi }{76}{example.B.1}\protected@file@percent }
\newlabel{ex:Varc1}{{B.1}{76}{}{example.B.1}{}}
\newlabel{ex:Varc1@cref}{{[example][1][2]B.1}{[1][76][]76}{}{}{}}
\@writefile{loe}{\contentsline {proposition}{\ifthmt@listswap Proposition~B.2\else \numberline {B.2}Proposition\fi }{76}{proposition.B.2}\protected@file@percent }
\newlabel{prop:Varchenko}{{B.2}{76}{}{proposition.B.2}{}}
\newlabel{prop:Varchenko@cref}{{[proposition][2][2]B.2}{[1][76][]76}{}{}{}}
\@writefile{loe}{\contentsline {example}{\ifthmt@listswap Example~B.3\else \numberline {B.3}Example\fi }{76}{example.B.3}\protected@file@percent }
\newlabel{ex:Varc2}{{B.3}{76}{}{example.B.3}{}}
\newlabel{ex:Varc2@cref}{{[example][3][2]B.3}{[1][76][]76}{}{}{}}
\citation{Varchenko}
\citation{OrTe}
\citation{OrTe}
\bibstyle{alpha}
\bibdata{loop_ampl}
\bibcite{AGPR}{AGPR24}
\bibcite{abcgpt}{AHBC{$^{+}$}16}
\bibcite{ABL}{AHBL17}
\bibcite{AHCC}{AHCC10}
\bibcite{AHT}{AHT14}
\bibcite{AHTT}{AHTT18}
\bibcite{AlMa}{AM07}
\bibcite{Akop_Tar}{AT08}
\bibcite{BCFW}{BCFW05}
\bibcite{BHL}{BHL16}
\bibcite{BlKa}{BK23}
\bibcite{BNR}{BNR24}
\@writefile{loe}{\contentsline {remark}{\ifthmt@listswap Remark~B.4\else \numberline {B.4}Remark\fi }{77}{remark.B.4}\protected@file@percent }
\newlabel{eq:Varchenko:dlog_Phi}{{B.1}{77}{T-embeddings~with~prescribed~boundary and positroid hyperplane arrangements}{equation.B.1}{}}
\newlabel{eq:Varchenko:dlog_Phi@cref}{{[equation][1][2]B.1}{[1][77][]77}{}{}{}}
\@writefile{loe}{\contentsline {problem}{\ifthmt@listswap Problem~B.5\else \numberline {B.5}Problem\fi }{77}{problem.B.5}\protected@file@percent }
\@writefile{toc}{\contentsline {section}{\tocsection {Appendix}{}{References}}{77}{section*.21}\protected@file@percent }
\bibcite{Chelkak_ICM}{Che18}
\bibcite{Chelkak_s_emb}{Che24}
\bibcite{CHY1}{CHY14}
\bibcite{CLR2}{CLR21}
\bibcite{CLR1}{CLR23}
\bibcite{CheRa}{CR24}
\bibcite{CheSmi}{CS12}
\bibcite{DFLP}{DFLP19}
\bibcite{DHKS}{DHKS10}
\bibcite{Dubedat}{Dub11}
\bibcite{ElHu}{EH15}
\bibcite{Eckmann_Hilton}{EH62}
\bibcite{ELPTSBW}{EZLP{$^{+}$}23}
\bibcite{ELT}{EZLT25}
\bibcite{FL}{FL23}
\bibcite{Farber_Postnikov}{FP16}
\bibcite{applets}{Gal}
\bibcite{origami2}{Gal26}
\bibcite{GKL1}{GKL22}
\bibcite{GL_parity}{GL20}
\bibcite{GP_Ising}{GP20}
\bibcite{Hodges}{Hod13}
\bibcite{Hull}{Hul02}
\bibcite{Huang_Wen}{HW14}
\bibcite{Huang_Wen_Xie}{HWX14}
\bibcite{HZ_notes}{HZ18}
\bibcite{Karp}{Kar19}
\bibcite{Kasteleyn}{Kas61}
\bibcite{Kawasaki}{Kaw89}
\bibcite{Kenyon}{Ken02}
\bibcite{Kenyon_lectures}{Ken09}
\bibcite{KLRR}{KLRR22}
\bibcite{KLS}{KLS13}
\bibcite{Kenyon_Sheffield}{KS04}
\bibcite{KW}{KW19}
\bibcite{KWZ}{KWZ20}
\bibcite{Lam_dimers}{Lam15}
\bibcite{LamCDM}{Lam16}
\bibcite{Lam_moduli}{Lam25}
\bibcite{Lovasz_Plummer}{LP86}
\bibcite{LPW}{LPW23}
\bibcite{Lus2}{Lus94}
\bibcite{Suho_rank}{MO20}
\bibcite{MuSp}{MS17}
\bibcite{OPT}{OPT25}
\bibcite{OrTe}{OT95}
\bibcite{Pak_book}{Pak10}
\bibcite{Parisi_thesis}{Par23}
\bibcite{Pos}{Pos06}
\bibcite{PSBW}{PSBW23}
\bibcite{Rietsch_alg}{Rie99}
\bibcite{RhSk}{RS05}
\bibcite{Skandera}{Ska04}
\bibcite{Smirnov_cluster}{Smi10}
\bibcite{SpeyerVariations}{Spe16}
\bibcite{Stanley_hyp}{Sta07}
\bibcite{Talaska}{Tal08}
\bibcite{Tasmuratov}{Tas74}
\bibcite{TF_exact}{TF61}
\bibcite{Valentine}{Val45}
\bibcite{Varchenko}{Var95}
\newlabel{tocindent-1}{0pt}
\newlabel{tocindent0}{63.44928pt}
\newlabel{tocindent1}{71.66179pt}
\newlabel{tocindent2}{0pt}
\newlabel{tocindent3}{0pt}
\gdef \@abspage@last{80}

